Almost Envy-free Allocation of Indivisible Goods: A Tale of Two Valuations

The existence of $\textsf{EFX}$ allocations stands as one of the main challenges in discrete fair division.In this paper, we present symmetrical results on the existence of $\textsf{EFX}$ and its approximate variations for two distinct valuations: restricted additive valuations and $(p,q)$-bounded valuations introduced by Christodoulou \etal \cite{christodoulou2023fair}. In a $(p,q)$-bounded instance, each good has relevance for at most $p$ agents, and any pair of agents shares at most $q$ common relevant goods. We show that instances with $(\infty,1)$-bounded valuations admit $\textsf{EF2X}$ allocations and $\textsf{EFX}$ allocations with at most $\lfloor {n}/{2} \rfloor - 1$ discarded goods, mirroring results for the restricted additive setting \cite{akrami2022ef2x}. We also present ${({\sqrt{2}}/{2})\textsf{-EFX}}$ algorithms for both restricted additive and $(\infty,1)$-bounded subadditive settings. The symmetry of these results suggests these valuations share symmetric structures. Building on this, we propose an $\textsf{EFX}$ allocation for restricted additive valuations when $p=2$ and $q=\infty$. To achieve these results, we further develop the rank concept introduced by Farhadi \etal \cite{farhadi2021almost} and introduce several new concepts such as virtual value, rankpath, and root, which advance the overall understanding of $\textsf{EFX}$ allocations. In addition, we suggest an updating rule based on the virtual values which we believe will lead to broader and more generalized results on $\textsf{EFX}$.

==> src/app5.tex <==
\section{Missing Proofs of Section \ref{sec:5}}

\iffalse
%\subsection{Schematic Overview of the Updating Rules}
 \label{sour5}
\begin{minipage}{7cm}
\begin{tcolorbox}[colback=blue!5,coltitle=white,colframe=blue!50!black,
	title= \textbf{Update Rule $1$}]
	\begin{itemize}
		\item $\malloc$ satisfies Property \ref{prop:2}. 
		\item \label{prec_1} There exists a good $ \good \in \malloc_{0}$ and an agent $i$ such that $\valu_i(\good) \neq 0$. 	\end{itemize}
	\vspace{1cm}
\tcblower
	\begin{itemize}
		\item $\malloc'_j = \begin{cases}
			\malloc_j & j \neq \{i,0\}\\
			\malloc_i \cup \good & j=i \\
			\malloc_0 \setminus \good & j=0
		\end{cases}$ 
		\item Run envy elimination
	\end{itemize}
\end{tcolorbox}
\end{minipage}
\begin{minipage}{9.4cm}
\begin{tcolorbox}[colback=blue!5,coltitle=white,colframe=blue!50!black,
	title= \textbf{Update Rule $2$}]
	\begin{itemize}
		\item Rule 1 is not applicable. 
		\item $\malloc$ satisfies Property \ref{prop:2}. 
		\item There is a path $i_1 \rightarrow \ldots \rightarrow i_k$ in $G_{\sqrt{2},\malloc}$ such that $i_1$ is a source in $G_{\sqrt{2},\malloc}$ and $\sqrt{2}\valu_{i_k}(\malloc_{i_k}) < \valu_{i_k}(\malloc_0)$. 
	\end{itemize}
	\tcblower
	\begin{itemize}
		\item $\malloc'_j = \begin{cases}
			\malloc_{i_{l+1}} & j = i_l \mbox{ for } 1 \le l < k\\
			\relevant_{i_k}(\malloc_0) & j = i_k\\
			\malloc_0 \cup \malloc_{i_1} \setminus \relevant_{i_k}(\malloc_0) & j = 0\\
			\malloc_j & \mbox{o/w}
		\end{cases}$
		\item Run envy elimination
	\end{itemize}
\end{tcolorbox}
\end{minipage}
\begin{tcolorbox}[colback=blue!5,coltitle=white,colframe=blue!50!black,
	title= \textbf{Final Step}]
	\begin{itemize}
		\item Rule 1, and Rule 2 are not applicable.
		\item $\malloc$ satisfies Property \ref{prop:2}. 
	\end{itemize}
\tcblower
	\begin{itemize}
		\item Suppose agent $i$ with minimum $\valu(\malloc_i)$. 
		\item $\malloc'_j = \begin{cases}
			\malloc_j & j \in [n] \setminus \{i\}\\
			\malloc_j \cup \malloc_0 & j = i
		\end{cases}$
	\end{itemize}
\end{tcolorbox}
% \newpage
\fi

Lemma \ref{lem:phi} helps us prove some of our claims in Section \ref{sec:5}. A Lemma similar to Lemma \ref{lem:phi} has been previously proved by Akrami \etal.\cite{akrami2022ef2x}. For completeness, here we restate and prove this lemma.
\begin{lemma}\label{lem:phi}
	Let $\alloc$ and $\alloc'$ be two allocations. Define:
	\begin{align*}
		A = \{i | \alloc_i \neq \alloc'_i\} \\
		x = \min_{i \in A}(\valu(\alloc_i)) \\
		x' = \min_{i \in A}(\valu(\alloc'_i)).
	\end{align*}
	Assume the following conditions hold:
	\begin{itemize}
		\item $x < x'$,
		\item There is only one source agent in $A$ in $G{\beta,\alloc}$,
		\item If $i$ is the source agent in $A$, then $\valu(\alloc_i)=x$.
	\end{itemize}
	Then, $\phi(\alloc) < \phi(\alloc')$.
\end{lemma}
\begin{proof}
	Denote the sources of $G_{\beta, \alloc}$ by $s_1, s_2, \ldots, s_k$ and the sources of $G_{\beta, \alloc'}$ by $s'_1, s'_2, \ldots, s'_{k'}$. Then:
	\begin{align*}
		\phi(\alloc) = \big[ \valu(\alloc_{s_1}),\valu(\alloc_{s_2}),\ldots, \valu(\alloc_{s_k}),\infty \big], \\
		\phi(\alloc') = \big[ \valu(\alloc'_{s'_1}),\valu(\alloc'_{s'_2}),\ldots, \valu(\alloc'_{s'_{k'}}),\infty \big].
	\end{align*}
	Since agent $i$ is a source in $G_{\beta, \alloc}$, we can assume without loss of generality that there exist an index $l$ such that $s_l = i$, and $\valu(\alloc_{s_l}) \neq \valu(\alloc{s_{l+1}})$. (we can reorder same values in $\phi$ to satisfy this condition). We show that for every $l' < l$ we have $\phi(\alloc)_{l'} = \phi(\alloc')_{l'}$ and for $l$ we have $\phi(\alloc)_l < \phi(\alloc')_l$. 
	\begin{itemize}
		\item For every $l' < l$, we claim that $s_{l'}$ remains a source in $G_{\beta, \alloc'}$. To prove this, we show that for every agent $j$ we have $\valu_j(\alloc'_{s_{l'}}) < \beta \valu_j(\alloc'_j)$. If $j \notin A$, our claimi is trivial since $s_{l'}$ is a source in $G_{\beta, \alloc}$. If $j \in A$, we have: 
		\begin{align*}
			\valu_j(\alloc'_{s_{l'}}) &\le \valu(\alloc'_{s_{l'}}) &\\
			&= \valu(\alloc_{s_{l'}}) &\text{$s_{l'} \notin A$}\\
			&\le x &\text{$l' < l$}, \\
			&< x' \\
			&\le \valu(\alloc'_j) &\text{$j \in A$},\\
			&= \valu_j(\alloc'_j) &\\
			&\le \beta \valu_j(\alloc'_j). 
		\end{align*}
		Therefore $j$ does not $\beta$-envy $s_{l'}$ in $\alloc'$ and $\phi(\alloc)_{l'} = \phi(\alloc')_{l'}$. 
		
		\item To prove $\phi(\alloc)_l < \phi(\alloc')_l$, we need to show that for any source agent $j$ in $G_{\beta, \alloc'}$ 
		such that $j \notin \{s_1, s_2, \dots, s_{l - 1}\}$ we have $\valu(\alloc'_j) > x = \phi(\alloc)_l$. 
		We have three cases. 
		The first case is $j \in A$. In this case we have: 
		\begin{align*}
			\phi(\alloc)_l &= x &\\
			& < x'\\
			&\le \valu(\alloc'_j) &\text{$j \in A$}. 
		\end{align*}
		In the second case we have $j \notin A$ and $j$ is also a source in $G_{\beta, \alloc}$. In this case we have: 
		\begin{align*}
			\phi(\alloc)_l &= x &\\
			&< \valu(\alloc_j) &\text{$j \notin {s_1, s_2, \dots, s_{l - 1}}$},\\
			&= \valu(\alloc'_j) &\text{$j \notin A$}. 
		\end{align*}
		In the last case we have $j \notin A$ and $j$ is not a source in $G_{\beta, \alloc}$. We know there exists another agent $j' \in A$ such that $j'$ $\beta$-envies agent $j$ in $G_{\beta, \alloc}$. Therefore we have: 
		\begin{align*}
			\phi(\alloc)_l &= x &\\
			&< \sqrt{2} x &\\
			& \le\sqrt{2} \valu(\alloc_{j'}) &\text{$j' \in A$},\\
			&< \valu(\alloc_j) &\text{$j'$ envies $j$ in $\alloc$},\\
			&= \valu(\alloc'_j) &\text{$j \notin A$}. 
		\end{align*}
	\end{itemize}
	Hence, $\phi(\alloc')_l$ is replaced with an agent with a larger value, or $\phi(\alloc')_l = \infty$. 
	
\end{proof}.


\begin{proof}[of \cref{lem:2}]
	By definition of the process, Property \ref{prop:2} trivially holds. To show that $\phi(\malloc) \leq \phi(\malloc')$, note that the envy elimination process may involve multiple updates. We show that after each update, the value of $\phi$ does not decrease. Consider an allocation $\malloc$ where, for some agents $i$ and $j$, we have $\sqrt{2}\valu_i(\malloc_i) < \valu_i({\malloc_j / \{\good\}})$. Let $\malloc''$ be the allocation after the update, which means $\malloc''$ is identical to $\malloc$ except that good $\good$ is transferred from the bundle of agent $j$ to the pool. Note that agent $j$ is neither a source before the update nor becomes a source after, since agent $i$ $\sqrt{2}$-envies agent $j$ both before and after the process. The only change in the source nodes happens when agent $j$ starts to $\sqrt{2}$-envy some source node after the process. Therefore, the set of sources in $G_{\sqrt{2}, \malloc}$ is a subset of the set of sources $G_{\sqrt{2}, \malloc''}$. Therefore, by definition of $\phi(\cdot)$, we have $\phi(\malloc) \leq \phi(\malloc'')$, and  consequently, $\phi(\malloc) \leq \phi(\malloc')$.
\end{proof}

\begin{proof}[of \cref{lem:511}]
	The only agent whose value for her bundle is changed is agent $i$, and the allocated good $\good$ is relevant to agent $i$. Therefore, Property \ref{prop:2} holds. Furthermore, $\valu(\malloc'_i) > \valu(\malloc_i)$ and  by Lemma \ref{lem:phi} we have $\phi(\malloc) < \phi(\malloc')$. 
\end{proof}

\begin{proof}[of \cref{lem:521}]
	Given that agent 
	$i$
	selects only relevant goods from the pool, we have $\valu_i(\malloc'_i) = \valu({\malloc'_i})$. Furthermore, according to Lemma \ref{lem:12}, for every edge $i_1 \rightarrow i_2$ in the path from $j$ to $i$, we have  $\valu_{i_1}(\malloc'_{i_2}) = \valu(\malloc'_{i_2})$. Consequently, Property \ref{prop:2} remains valid after the update.
	To prove $\phi(\malloc) < \phi(\malloc')$, we utilize Lemma \ref{lem:phi}. Considering $A,x,x'$ in the statement of Lemma \ref{lem:phi} we proceed with: 
	\begin{align*}
		A &= \mbox{Agents in the path from $j$ to $i$ } \\
		x &= \min_{i' \in A}(\valu(\alloc_{i'})) = \valu(\malloc_j) \\
		x' &= \min_{i' \in A}(\valu(\alloc'_{i'}))
	\end{align*}
	Also, since for agent $i$, $\valu(\malloc_j) < \invsq\valu(\malloc_i) 
	< \valu(\malloc'_i),
	$
	and for every other agent $k \in A$, $\valu(\malloc_j) < \invsq\valu(\malloc_{k})$, we have $x < x'$.  
	Finally, agent $j$ is a source in $G_{\sqrt{2}, \malloc}$ and therefore, $x = \valu(\malloc_j)$. Thus, all conditions of Lemma \ref{lem:phi} are satisfied, which implies $\phi(\malloc) < \phi(\malloc')$.
\end{proof}

\begin{proof}[of \cref{thm:fstep}]
	Let $\malloc$ be the allocation before the final step.
	First, note that agent $1$ is a source in $G_{\sqrt{2}, \malloc}$. We prove that after this allocation, no-one will $\sqrt{2}$-envy $\malloc^*_1$. As a contradiction, 
	suppose agent $i$ $\sqrt{2}$-envies agent $1$. Since agent $1$ was a source, agent $i$ did not $\sqrt{2}$-envy him before the final step. This means that the pool has a non-zero value for agent $i$, and given the fact that Rule 1 was not applicable, agent $i$ is not a source. Now, suppose that agent $j$ is a source that has a path to $i$. We have
	\begin{align*}
		\valu_i(\malloc^*_1) &= \valu(\malloc_1) + \valu_i(\malloc_0) \\
		&\leq  \valu(\malloc_j) + \valu_i(\malloc_0) &\valu(\malloc_1) \leq\valu(\malloc_j)  \\
		&\leq \frac{\sqrt{2}}{2}\valu(\malloc_i)  + \valu_i(\malloc_0) & \mbox{ $j$  has a path to $i$ in }G_{\sqrt{2},\malloc}\\
		&\leq \frac{\sqrt{2}}{2}\valu(\malloc_i)  + \frac{\sqrt{2}}{2}\valu(\malloc_i) & \mbox{$i$ does not $\sqrt{2}$-envy $\malloc_0$}\\
		&\leq \sqrt{2}\valu(\malloc_i). 
	\end{align*}
	But this contradicts the fact that agent $i$ does not $\sqrt{2}$-envy agent $j$ before the final step.
\end{proof} 

==> src/app6.tex <==
\section{Missing Proofs of Section \ref{sec:eh}}

\iffalse
\begin{minipage}{8.2cm}
\begin{tcolorbox}[colback=blue!5,coltitle=white,colframe=blue!50!black,
	title= \textbf{Update Rule $1$}]
	\begin{itemize}
		\item $(\malloc, \core)$ satisfies \ref{thresh-ef}, \ref{one-item}  and \ref{relevant-items}.
		\item \label{prec_1}$ \exists i, \good \in \alloc_{0}$ s.t $\valu_i(\malloc_i,\core)<\valu_i(\good)$. 	\end{itemize}
\tcblower
	\begin{itemize}
		\item $\malloc'_j = \begin{cases}
			\malloc_j & j \in [n] \setminus \{i,0\}\\
			\{\good\} & j=i \\
			\malloc_0 \cup \alloc_i & j=0
		\end{cases}$
		\item  $\core' = \core \setminus \{i\}$.
	\end{itemize}
\end{tcolorbox}
\end{minipage}
\begin{minipage}{8.2cm}
\begin{tcolorbox}[colback=blue!5,coltitle=white,colframe=blue!50!black,
	title= \textbf{Update Rule $2$}]	
	\begin{itemize}
		\item Rule 1 is not applicable. 
		\item $(\alloc, \core)$ satisfies \ref{thresh-ef}, \ref{one-item}  and \ref{relevant-items}.
		\item \label{prec_2}$ \exists \good \in \alloc_{0},i \in \core$ s.t. $\valu_i(\good)>0$. 	
	\end{itemize}
\tcblower
	\begin{itemize}
		\item $\malloc'_j = \begin{cases}
			\malloc_j & j \in [n] \setminus \{i\}\\
			\malloc_j \cup \{\good\} & j=i 
		\end{cases}$
		\item  $\core' = \core $.
	\end{itemize}
\end{tcolorbox}
\end{minipage}
\begin{minipage}{8.5cm}
\begin{tcolorbox}[colback=blue!5,coltitle=white,colframe=blue!50!black,
	title= \textbf{Update Rule $3$}]
	\begin{itemize}
		\item $(\alloc, \core)$ satisfies \ref{thresh-ef}, \ref{one-item}  and \ref{relevant-items}.
		\item \label{prec_3}There is a cycle $i_1  \rightarrow \ldots, \rightarrow i_k \rightarrow i_1$ in $H_\sigma$. 	
	\end{itemize}
\tcblower
	\begin{itemize}
		\item $\malloc'_j = \begin{cases}
			\relevant_{i_l}(\malloc_{i_{l\%k+1}}) & j=i_\ell \mbox { for }  1 \leq l \leq k.\\
						\malloc_j & \mbox{o/w}\\
			 
		\end{cases}$
		\item  $\core' = (\core \setminus \{i_1,\ldots,i_k\}) \cup \{i_l \mid i_{l \%k +1} \in \core \} $.
	\end{itemize}
\end{tcolorbox}
\end{minipage}
\begin{minipage}{7.9cm}
\begin{tcolorbox}[colback=blue!5,coltitle=white,colframe=blue!50!black,
	title= \textbf{Update Rule $4$}]
	\begin{itemize}
		\item $(\alloc, \core)$ satisfies \ref{thresh-ef}, \ref{one-item}  and \ref{relevant-items}.
		\item Rule 1 is not applicable.
		\item $\exists i \notin \core$ s.t. $\valu_i(\malloc_i) < \sqrt{2} \cdot \valu_i(\malloc_0)$.
	\end{itemize}
\tcblower
	\begin{itemize}
		\item $\malloc'_j = \begin{cases}
			\malloc_j & j \in [n] \setminus \{i\}\\
			\relevant_j(\malloc_0) & j = i
		\end{cases}$
		\item  $\core' = \core \cup \{i\}$
	\end{itemize}
\end{tcolorbox}
\end{minipage}
\begin{tcolorbox}[colback=blue!5,coltitle=white,colframe=blue!50!black,
	title= \textbf{Final Step}]
	\begin{itemize}
		\item $(\alloc, \core)$ satisfies \ref{thresh-ef}, \ref{one-item},  and \ref{relevant-items}.
		\item Rule 1 , Rule 2, Rule 3, and Rule 4 are not applicable.
	\end{itemize}
\tcblower
	\begin{itemize}
		\item Find an agent $i$ with no incoming edge in $H_\conf$.
		\item $\malloc'_j = \begin{cases}
			\malloc_j & j \in [n] \setminus \{i\}\\
			\malloc_j \cup \malloc_0 & j = i
		\end{cases}$
	\end{itemize}
\end{tcolorbox}

% \newpage

\fi

\begin{proof}[of \cref{same-virtual-value}]
	We distinguish among three cases:
	
	\textbf{Case 1 ($j \notin P$):} We have $\rupp_j = \rank_i(\malloc)$ and $\malloc'_j = \malloc_j$. This implies: $$\virtualvalue_j(\malloc) = \frac{\valu_j(\malloc_j)}{\rank_i(\malloc)} = \frac{\valu_j(\malloc'_j)}{\rupp_j}.$$
	
	\textbf{Case 2 ($j \rightarrow k \in P$):} After shifting the bundles through $P$, agent $j$ receives the bundle of agent $k$. Furthermore, since $P$ is the rankpath of agent $i$, by Observation \ref{obs:rankpath} we have $\rank_k(\malloc) = \rank_j(\malloc)  \frac{\valu_j(\malloc_k)}{\valu_j(\malloc_j)}$. Hence:
	\begin{align*}
		\frac{\valu_j(\malloc'_j)}{\rupp_j} &= \frac{\valu_j(\malloc_k)}{\rank_k(\malloc)} & \mbox{$\malloc'_j = \malloc_k$ and $\rupp_j = \rank_k(\malloc)$} \\
		&= \frac{\valu_j(\malloc_j)}{\rank_j(\malloc)} = \virtualvalue_j(\malloc) & \mbox{Observation \ref{obs:rankpath}}.
	\end{align*}
	
	\textbf{Case 3 ($j = i$):} Since $\malloc'_i = \hat{\malloc_0}$, we have:
	\begin{align*}
		\frac{\valu_i(\malloc'_i)}{\rupp_i} &= \frac{\valu_i(\hat{\malloc_0})}{\rupp_i} & \mbox{$\malloc'_i = \hat{\malloc_0}$} \\
		&= \frac{\valu_i(\hat{\malloc_0})}{\frac{\valu_i(\hat{\malloc_0})}{\virtualvalue_i(\malloc)}} = \virtualvalue_i(\malloc) & \mbox{$\rupp_i = \frac{\valu_i(\hat{\malloc_0})}{\virtualvalue_i(\malloc)}$}.
	\end{align*}
\end{proof}

\begin{proof}[of \cref{rupp-satisfies-rank-property}]
	In order to show that for every agents $j$ and $k$, $\rupp_j w_{\malloc'}(j, k) \le \rupp_k$, we distinguish three cases:
	
	\textbf{Case 1 ($k \notin P$):} The bundle of agent $k$ remains the same as it was before. Therefore:
	\begin{align*}
		\rupp_j w_{\malloc'}(j, k) &= \frac{\rupp_j}{\valu_j(\malloc'_j)} \valu_j(\malloc'_k) & \mbox{Definition \ref{weighted-envy-def}} \\
		&= \frac{\valu_j(\malloc'_k)}{\virtualvalue_j(\malloc)} & \mbox{Lemma \ref{same-virtual-value}} \\
		&= \frac{\valu_j(\malloc_k)}{\virtualvalue_j(\malloc)} & \mbox{$\malloc'_k = \malloc_k$} \\
		&= \rank_j(\malloc) \frac{\valu_j(\malloc_k)}{\valu_j(\malloc_j)} & \mbox{Definition \ref{virtual-value-def}}\\
		&\le \rank_k(\malloc) & \mbox{ Property \ref{q1-no-greater-1-cycle}} 
		\\
		&= \rupp_k. & \mbox{Equation \eqref{rank-upperbound-def}}
	\end{align*}
	
	\textbf{Case 2 ($k \rightarrow l \in P$):} Agent $k$ receives the bundle of agent $l$. Additionally, by Equation \eqref{rank-upperbound-def}, we have $\rupp_k = \rank_l(\malloc)$. Therefore:
	
	\begin{align*}
		\rupp_j w_{\malloc'}(j, k) &= \frac{\rupp_j}{\valu_j(\malloc'_j)} \valu_j(\malloc'_k) & \mbox{Definition \ref{weighted-envy-def}} \\
		&= \frac{\valu_j(\malloc'_k)}{\virtualvalue_j(\malloc)} & \mbox{Lemma \ref{same-virtual-value}} \\
		&= \frac{\valu_j(\malloc_l)}{\virtualvalue_j(\malloc)} & \mbox{$\malloc'_k = \malloc_l$} \\
		&= \rank_j(\malloc) \frac{\valu_j(\malloc_l)}{\valu_j(\malloc_j)} & \mbox{Definition \ref{virtual-value-def}}\\
		&\le \rank_l(\malloc) & \mbox{$\malloc$ satisfies Property \ref{q1-no-greater-1-cycle}} 
		\\
		&= \rupp_k & \mbox{Equation \eqref{rank-upperbound-def}}.
	\end{align*}
	
	\textbf{Case 3 ($k = i$):} Agent $i$ receives $\hat{\malloc_0}$. Note that since $i$ has the maximum value of $\frac{v_i(\hat{\malloc_0})}{\virtualvalue_i(\malloc)}$ we have $\frac{v_j(\hat{\malloc_0})}{\virtualvalue_j(\malloc)} \le \frac{v_i(\hat{\malloc_0})}{\virtualvalue_i(\malloc)}$. This implies:
	
	\begin{align*}
		\rupp_j w_{\malloc'}(j, i) &= \frac{\rupp_j}{\valu_j(\malloc'_j)} \valu_j(\malloc'_i) & \mbox{Definition \ref{weighted-envy-def}} \\
		&= \frac{\valu_j(\malloc'_i)}{\virtualvalue_j(\malloc)} & \mbox{Lemma \ref{same-virtual-value}} \\
		&= \frac{\valu_j(\hat{\malloc_0})}{\virtualvalue_j(\malloc)} & \mbox{$\malloc'_i = \hat{\malloc_0}$} \\
		&\le \frac{v_i(\hat{\malloc_0})}{\virtualvalue_i(\malloc)} &\mbox{ $\frac{v_i(\hat{\malloc_0})}{\virtualvalue_i(\malloc)}$ is maximum} \\
		&= \rupp_i & \mbox{Equation \eqref{rank-upperbound-def}}.
	\end{align*}
\end{proof}

\begin{proof}[of \cref{virtual-value-increases}]
	Lemma \ref{rupp-satisfies-rank-property} ensures that for every agents $j$ and $k$ we have $\rupp_j w_{\malloc'}(j, k) \le \rupp_k$. According to Lemma \ref{upper-bound-no-cycle}, this guarantees $G_{\malloc'}$ does not have any cycle whose total product of the edge weights is strictly greater than $1$. Additionally, by Lemma \ref{rank-upper-bound}, for each agent $j$, we have $\rank_j(\malloc') \le \rupp_j$ and Lemma \ref{same-virtual-value} implies that $\virtualvalue_j(\malloc) = \frac{\valu_j(\malloc'_j)}{\rupp_j}$. Consequently, we have $\virtualvalue_j(\malloc') = \frac{\valu_j(\malloc'_j)}{\rank_j(\malloc')} \ge \frac{\valu_j(\malloc'_j)}{\rupp_j} = \virtualvalue_j(\malloc)$.
\end{proof}

\begin{proof}[of \cref{no-virtual-se}]
	We show that every agent $j$ does not virtually strongly envy another agent $k$. If $k \ne i$, there exists a (not necessarily different from $k$) agent $l$ such that $\malloc'_k = \malloc_l$. Therefore, for every good $g \in \malloc'_k = \malloc_l$ we have:
	\begin{align*}
		\virtualvalue_j(\malloc') &\ge \virtualvalue_j(\malloc) & \mbox{Lemma \ref{virtual-value-increases}} \\
		&\ge \valu_j(\malloc_l \setminus \{g\}) & \mbox{$\malloc$ satisfies Property \ref{q1-virtually-efx}} \\
		&= \valu_j(\malloc'_k \setminus \{g\}) & \mbox{$\malloc'_k = \malloc_l$}.
	\end{align*}
	Additionally, for agent $i$, we know that $i$ receives $\hat{\malloc_0}$, which is the minimal subset that is virtually envied by at least one agent. Hence, $j$ does not virtually strongly envy agent $i$.
\end{proof}

\begin{proof}[of \cref{lem:q1-relevant-goods}]
	If $j \notin P$, since $\malloc'_j = \malloc_j$, the property trivially holds. Additionally, since $\hat{\malloc_0}$ is minimal, all the goods in $\malloc'_i$ are relevant to agent $i$. Now, we only need to show that for every agent $j \rightarrow k \in P$, all the goods in $\malloc'_j = \malloc_k$ are relevant to agent $j$. Assume by contradiction that there exists a good $g \in \malloc_k = \malloc'_j$ that is not relevant to agent $j$. Then, we have:
	\begin{align*}
		\valu_j(\malloc_k \setminus \{g\}) &= \valu_j(\malloc_k) & \mbox{$g$ is not relevant to $j$} \\
		&= \valu_j(\malloc_j) w_\malloc(j, k) & \mbox{Definition \ref{weighted-envy-def}} \\
		&= \valu_j(\malloc_j) \frac{\rank_k(\malloc)}{\rank_j(\malloc)} & \mbox{Observation \ref{obs:rankpath}} \\
		&= \virtualvalue_j(\malloc) \rank_k(\malloc) & \mbox{Definition \ref{virtual-value-def}} \\
		&> \virtualvalue_j(\malloc) & \mbox{$\rank_k(\malloc) > 1$}.
	\end{align*}
	Therefore, agent $j$ virtually strongly envies $k$ in allocation $\malloc$. This contradicts the fact that $\malloc$ satisfies Property \ref{q1-virtually-efx}.
\end{proof}

\begin{proof}[of \cref{nsw-increases}]
	Since the bundle of agents that are not in $P$ is still the same as before, it is sufficient to show that the product of valuation of agents in path $P$ increases.
	\begin{align*}
		\prod_{j \in P} \valu_j(\malloc'_j) &= \valu_i(\hat{\malloc_0}) \prod_{j \rightarrow k \in P} \valu_j(\malloc_k) & \mbox{Bundles are shifted through path $P$} \\
		&> \virtualvalue_i(\malloc) \prod_{j \rightarrow k \in P} \valu_j(\malloc_k) &\mbox{$\valu_i(\hat{\malloc_0}) > \virtualvalue_i(\malloc)$} \\
		&= \frac{\valu_i(\malloc_i)}{\rank_i(\malloc)} \prod_{j \rightarrow k \in P} \valu_j(\malloc_k) &\mbox{Definition \ref{virtual-value-def}} \\
		&= \frac{\valu_i(\malloc_i)}{\rank_i(\malloc)} \prod_{j \rightarrow k \in P} \valu_j(\malloc_j) w_\malloc(j, k) &\mbox{Definition \ref{weighted-envy-def}} \\
		&= \frac{\rank_i(\malloc)}{\rank_i(\malloc)} \prod_{j \in P} \valu_j(\malloc_j) & \mbox{$P$ is rankpath of $i$} \\
		&= \prod_{j \in P} \valu_j(\malloc_j).
	\end{align*}
	Therefore $\nsw(\malloc') > \nsw(\malloc)$.
\end{proof}

\begin{proof}[of \cref{thm72}]
	First we show that for every agents $j \in \sagents$ and $k \in \agents$, agent $k$ does not $\sqrt{2}$-envy agent $j$. Note that since $\malloc_k \subseteq \malloc^*_k$ we have $\valu_k(\malloc_k) \le \valu_k(\malloc^*_k)$. Additionally, since agent $j$ only receives the goods from the pool that are relevant to her, and the valuations are $(\infty, 1)$-bounded, at most one good in $\malloc^*_j$ is relevant to agent $k$. We denote this good by $g$. If $g \in \malloc_0$, since Rule 1 is not applicable $\valu_k(\malloc_k) \ge \virtualvalue_k(\malloc) \le \valu_k(g)$ and $k$ does not envy agent $j$; otherwise $g \in \malloc_j$, and since $\rank_j(\malloc) \le \sqrt{2}$ agent $k$ does not $\sqrt{2}$-envy $\malloc_j$. Hence, agent $k$ does not $\sqrt{2}$-envy agent $j$.
	
	Now, we need to prove that there is no agent $k \in \agents$ who $\sqrt{2}$-envies $\malloc^*_i$. In the case that $k \in \sagents$, since $k$ has picked all the goods from the pool which are relevant to her, agent $i$ does not receive any good that is relevant to agent $k$. Furthermore, since $\rank_i(\malloc) = 1$, agent $k$ does not envy agent $i$. For the case that $\rank_k(\malloc) > \sqrt{2}$, since Rule 1 is not applicable we have $\valu_k(\malloc_0) < \virtualvalue_k(\malloc) \le \invsq \valu_k(\malloc_k)$. Additionally, since $\malloc$ satisfies Property \ref{q1-no-greater-1-cycle} we have $\rank_k(\malloc) w_{\scriptscriptstyle \malloc}(k, i) \le \rank_i(\malloc)$, and since $\rank_i(\malloc) = 1$ and $\rank_k(\malloc) > \sqrt{2}$ we have $\valu_k(\malloc_i) \le \invsq \valu_k(\malloc_k)$. Therefore:
	\begin{align*}
		\valu_k(\malloc^*_i) &\le \valu_k(\malloc_i \cup \malloc_0) &\mbox{$\malloc^*_i \subseteq \malloc_i \cup \malloc_0$} \\
		&\le \valu_k(\malloc_i) + \valu_k(\malloc_0) & \mbox{Subadditivity} \\
		&\le \valu_k(\malloc_i) + \invsq \valu_k(\malloc_k) & \mbox{Rule 1 is not applicable} \\
		&\le \invsq \valu_k(\malloc_k) + \invsq \valu_k(\malloc_k) & \mbox{$\rank_i(\malloc) = 1$} \\
		&= \sqrt{2} \valu_k(\malloc_k).
	\end{align*}
	Hence, there is no agent $k$ that $\sqrt{2}$-envies agent $i$.
	
	It only remains to prove that for every agents $j$ and $k$ such that $\rank_k > \sqrt{2}$, agent $j$ does not strongly-envy agent $k$. Note that $\malloc$ satisfies Property \ref{q1-virtually-efx}, which means for every good $g \in \malloc_k$ we have $\virtualvalue_j(\malloc) \ge \valu_j(\malloc_k \setminus \{g\})$. Additionally, since $\rank_k(\malloc) > \sqrt{2}$, $k$ does not receive any good in the final step, i.e., $\malloc^*_k = \malloc_k$. Therefore $\valu_j(\malloc^*_j) \ge \virtualvalue_j(\malloc) \ge \valu_j(\malloc_k \setminus \{g\})$ and agent $j$ does not strongly envy agent $k$. 
	This completes the proof.
	%In conclusion, after the final step, there is no agent who $\sqrt{2}$-envies an agent $j$. %such that $\rank_j(\malloc) \le \sqrt{2}$ and there is no agent who strongly envies an agent $k$ such that $\rank_k(\malloc) > \sqrt{2}$.
	
	%for the agents whose rank is at most $\sqrt{2}$, no one will $\sqrt{2}$-envy them, and for the agents whose rank is strictly more than $\sqrt{2}$ no one will strongly envy them. Therefore, $\malloc^*$ is $\invsq$-$\efx$.
\end{proof}

==> src/app7.tex <==
\iffalse

\section{Overview of the Updating Rules of Section \ref{sec:7}} \label{sour7}

\begin{tcolorbox}[colback=blue!5,coltitle=white,colframe=blue!50!black,
	title= \textbf{Update Rule $1$}]
	\begin{itemize}
				\item $\malloc$ satisfies  Property \ref{prop:51}. 
		\item There is an agent $ i$ and a good  $\good \in \malloc_{0}$ such that $\valu_i(\malloc_i) < \valu_i(\good)$. 	
	\end{itemize}
\tcblower
	\begin{itemize}
		\item $\malloc'_j = \begin{cases}
			\{\good\} & j=i \\
			\malloc_0 \cup \malloc_i \setminus \{\good\} & j=0\\
			\malloc_j & \mbox{o/w}
		\end{cases}$
		\item Resolve all envy-cycles. 
	\end{itemize}
\end{tcolorbox}

\begin{tcolorbox}[colback=blue!5,coltitle=white,colframe=blue!50!black,
	title= \textbf{Update Rule $2$}]
	\begin{itemize}
		\item $\malloc$ satisfies Property \ref{prop:51}. 
		\item  There is a source agent $i$ and a good $\good \in \relevant{\malloc_{0}}{i}$.
	\end{itemize}	
	\tcblower
	\begin{itemize}
		\item $\malloc'_j = \begin{cases}
			\relevant{(\malloc_j \cup \{\good\})}{j} & j=i \\
			\malloc_0 \cup \malloc_i \setminus \relevant{\malloc_i}{j} & j=0\\
			\malloc_j & \mbox{o/w}
		\end{cases}$ 
		\item Resolve all envy-cycles. 	
	\end{itemize}
\end{tcolorbox}

\begin{tcolorbox}[colback=blue!5,coltitle=white,colframe=blue!50!black,
	title= \textbf{Update Rule $3$}]	
	\begin{itemize}
		\item $\malloc$ satisfies  \ref{prop:51}. 
		\item  $ \exists i, \good \in \malloc_{0}$ s.t.  $i$ is a source in $G_{1, \malloc}$ and $\forall j \neq i$ $\valu_j(\malloc_j) \geq \valu_j(\malloc_i \cup \{\good\})$. 
	\end{itemize}
\tcblower
	\begin{itemize}
		\item $\malloc'_j = \begin{cases}
			\malloc_i \cup \{\good\} & j=i \\
			\malloc_0 \setminus \{\good\} & j=0\\
			\malloc_j &\mbox{o/w}
		\end{cases}$ 
	\end{itemize}
\end{tcolorbox}

\begin{tcolorbox}[ colback=blue!5,coltitle=white,colframe=blue!50!black,
	title= \textbf{Update Rule $5$}]
	\begin{itemize}
		\item $\malloc$ satisfies \ref{prop:51}. 
		\item There are $l \ge 1$ distinct goods $\good_0, \good_1, \dots, \good_{l - 1} \in \malloc_0$, distinct sources $s'_0, s'_1, \dots s'_{l - 1}$ and distinct agents $t_1, t_2, \dots t_l$ such that $t_i \in \comp_\malloc(s'_i)$ and $t_{i + 1}$ is most envious agent of $\malloc_{s'_i} \cup \{\good_i\}$ for $0 \le i < l$. 
	\end{itemize}
\tcblower
	\begin{itemize}
		\item $\malloc'_j = \begin{cases}
			\malloc_j & j \mbox{ not in cycle }\\
			\mbox{Smallest subset of $\malloc_{s'_{i-1}} \cup \{\good_i\}$ which is envied by $t_i$}. & j=t_i \\
			\malloc_{j'} \mbox{ which $j'$ is $j$'s next agent in the cycle } & j \mbox{ in cycle but not $t_i$ }
		\end{cases}$ 
	\end{itemize}
\end{tcolorbox}

\begin{tcolorbox}[colback=blue!5,coltitle=white,colframe=blue!50!black,
	title= \textbf{Final step}]
	\begin{itemize}
		\item Rules 1, 2, 3, 4 and 5 are not applicable.
		\item $\malloc$ satisfies Property \ref{prop:51}. 
	\end{itemize}
\tcblower
	\begin{itemize}
		\item $\malloc'_j = \begin{cases}
			\malloc_j \cup \{\good_i\} & j  \mbox{ is an arbitrary non source agent in $\comp_\malloc(s_i)$ for } 1 \le i \le x\\
			\emptyset & j = 0\\
			\malloc_j & \mbox{\mbox{o/w}}
		\end{cases}$ 
	\end{itemize}
\end{tcolorbox}

\fi

==> src/app8.tex <==
\section{Missing Proofs of Section \ref{sec:8}}\label{sour8}

\iffalse 
\begin{minipage}{18cm}
	\begin{tcolorbox}[colback=blue!5,coltitle=white,colframe=blue!50!black,
		title= \textbf{Update Rule $1$}]
		\begin{itemize}
			\item $\malloc$ satisfies \ref{prop42} and \ref{prop43}. 
			\item There is an agent $i \in \agents$ and a good $\good \in \malloc_0$ such that $\rank_i(\malloc) = 1$ and $\good \in \relevant{\goods}{i, j}$ where $\malloc_i \subseteq \relevant{\goods}{i, j}$. 
		\end{itemize}
		\vspace{0.45cm}
		\tcblower
		\begin{itemize}
			\item $\malloc'_k = \begin{cases}
				\mbox{minimal subset of } \malloc_k \cup \good \mbox{ with value greater than } \valu(\malloc_k) & k = i\\
				\malloc_k & k \neq i
			\end{cases}$
		\end{itemize}
	\end{tcolorbox}
\end{minipage}

\begin{minipage}{18cm}
	\begin{tcolorbox}[colback=blue!5,coltitle=white,colframe=blue!50!black,
		title= \textbf{Update Rule $2$}]
		\begin{itemize}
			\item Rule 1 is not applicable. 
			\item $\malloc$ satisfies \ref{prop42} and \ref{prop43}. 
			\item There is a path $P = i_1 \rightarrow i_2 \rightarrow \ldots \rightarrow i$ in $G_{0, \malloc}$ such that $\virtualvalue_i(\malloc) \le \valu(\relevant{\malloc_0}{i, j})$ and $\virtualvalue_i(\malloc) \le \virtualvalue_j(\malloc)$ where $\malloc_i \subseteq \relevant{\goods}{i, j}$. 
		\end{itemize}
		\vspace{0.45cm}
		\tcblower
		\begin{itemize}
			\item $\malloc'_k = \begin{cases}
				\malloc_{i_{l + 1}} & k = i_l \in P, k \neq i\\
				
				\mbox{minimal subset of } \malloc_k \cup \good \mbox{ with value greater than } \virtualvalue_k(\malloc) & k = i\\
				
				\malloc_k & \mbox{o/w}
			\end{cases}$
		\end{itemize}
	\end{tcolorbox}
\end{minipage}

\begin{minipage}{18cm}
	\begin{tcolorbox}[colback=blue!5,coltitle=white,colframe=blue!50!black,
		title= \textbf{Update Rule $3$}]
		\begin{itemize}
			\item Rule 1 and 2 are not applicable. 
			\item $\malloc$ satisfies \ref{prop42} and \ref{prop43}. 
			\item There is an agent $i$ such that for every $j \in \agents$, we have $\valu_i(\malloc_j) = 0$. 
		\end{itemize}
		\vspace{0.45cm}
		\tcblower
		\begin{itemize}
			\item $\malloc'_k = \begin{cases}
				\relevant{\malloc_0}{k} & k = i, \valu_i(\malloc_i) < \valu_i(\malloc_0)\\
				\malloc_k & \mbox{o/w}
			\end{cases}$
			\item Remove $i$ from $\agents$ and $\malloc_i$ from $\malloc$. 
		\end{itemize}
	\end{tcolorbox}
\end{minipage}

\begin{minipage}{18cm}
	\begin{tcolorbox}[colback=blue!5,coltitle=white,colframe=blue!50!black,
		title= \textbf{Update Rule $4$}]
		\begin{itemize}
			\item Rule 1,2 and 3 are not applicable. 
			\item $\malloc$ satisfies \ref{prop42} and \ref{prop43}. 
			\item There is a cycle $C = i \rightarrow i_1 \rightarrow \ldots \rightarrow i_t \rightarrow i$ where $\rank_i(\malloc) = 1$. 
		\end{itemize}
		\vspace{0.45cm}
		\tcblower
		\begin{itemize}
			\item $\malloc'_k = \begin{cases}
				\malloc_k \cup \relevant{\malloc_0}{k} & k = i, \valu_i(\malloc_{i_1}) < \valu_i(\malloc_i \cup \malloc_0)\\
				\malloc_{l \% t + 1} & k \in C, \valu_i(\malloc_{i_1}) > \valu_i(\malloc_i \cup \malloc_0)\\
				\malloc_k & \mbox{o/w}
			\end{cases}$
			\item Remove $i$ from $\agents$ and $\malloc_i$ from $\malloc$. 
		\end{itemize}
	\end{tcolorbox}
\end{minipage}
\fi

\begin{proof}[of \cref{obs41}]
	Let $i_1 \rightarrow i_2 \rightarrow \dots \rightarrow i_k \rightarrow i$ be the rankpath of agent $i$ in $G_{\alloc}$. 
	
	\begin{align*}
		\rank_i(\alloc) &= w_{\scriptscriptstyle \alloc}(i_1, i_2) \times w_{\scriptscriptstyle \alloc}(i_2, i_3) \times \ldots \times w_{\scriptscriptstyle \alloc}(i_k, i) &\text{Definition \ref{weighted-envy-def}} \\
		&= \frac{\valu_{i_1}(\alloc_{i_2})}{\valu_{i_1}(\alloc_{i_1})} \times \frac{\valu_{i_2}(\alloc_{i_3})}{\valu_{i_2}(\alloc_{i_2})} \times \ldots \times  \frac{\valu_{i_k}(\alloc_{i})}{\valu_{i_k}(\alloc_{i_k})} & \\
		&= \frac{\valu(\alloc_{i_2})}{\valu(\alloc_{i_1})} \times \frac{\valu(\alloc_{i_3})}{\valu(\alloc_{i_2})} \times \ldots \times \frac{\valu(\alloc_{i})}{\valu(\alloc_{i_k})} &\text{Property \ref{prop42}} \\
		&= \frac{\valu(\alloc_i)}{\valu(\alloc_{i_1})}.
	\end{align*}
	
	Therefore $\virtualvalue_i(\alloc) = \frac{\valu(\alloc_i)}{\rank_i(\alloc_i)} = \valu(\alloc_i) \frac{\valu(\alloc_{i_1})}{\valu(\alloc_i)} = \valu(\alloc_{i_1}) = \valu(\alloc_{\roott{i}{\alloc}})$.	
\end{proof}

\begin{proof}[of \cref{path-virtual}]
	Let $r = \roott{i}{\alloc}$ and $r' = \roott{j}{\alloc}$. Since $r$ has a path to $j$, we have: 
	
	\begin{align*}
		\virtualvalue_j(\alloc) &= \valu(\alloc_{r'}) &\text{Observation \ref{obs41}} \\
		&\le \valu(\alloc_r) &\text{$r' = \roott{j}{\alloc}$} \\
		&= \virtualvalue_i(\alloc) &\text{Observation \ref{obs41}}. 
	\end{align*}
\end{proof}

\begin{proof}[of \cref{lem:prop43}]
	For every $j \in \agents$, we show that $\valu_j(\alloc_i \setminus \{\good\}) \le \virtualvalue_j(\alloc)$. Let $k$ be the corresponding agent of agent $i$. We have three cases $j = i$, $j = k$, and $j \notin \{i, k\}$. The first case is indeed the condition of the lemma. For the second case, we have: 
	
	\begin{align*}
		\valu_j(\alloc_i \setminus \{\good\}) &\le \valu(\alloc_i \setminus \{\good\}) &\\
		&\le \virtualvalue_i(\alloc) &\\
		&\le \virtualvalue_j(\alloc) &\text{Observation \ref{path-virtual}}\\
	\end{align*}
	
	And since $\alloc_i$ is relevant to only agents $i$ and $k$, for case $j \notin \{i, k\}$ we have $\valu_j(\alloc_i \setminus \{\good\}) = 0$ and the lemma trivially holds. 
\end{proof}

\begin{proof}[of \cref{lem:U81}]
	Given that \(\malloc'_i \subseteq \relevant{\goods}{i,j}\) and the other bundles remain unchanged, \(\malloc'\) satisfies Property \ref{prop42}.
	By Lemma \ref{lem:prop43}, to prove that $\malloc'$ satisfies Property \ref{prop43}, it's enough to show that for every remaining agent $k$ and $\good \in \malloc'_k$, we have $\valu(\malloc'_k \setminus \{\good\}) \le \virtualvalue_k(\malloc')$. There are two cases $k = i$ and $k \neq i$.
	Let \(k \neq i\) and a good \(\good \in \malloc'_k\) and \(r = \roott{k}{\malloc'}\). We have:
	
	\begin{align*}
		\valu(\malloc'_k \setminus \{\good\}) &= \valu(\malloc_k \setminus \{\good\}) & \text{$k \neq i$} \\
		&\le \virtualvalue_k(\malloc) &\text{Property \ref{prop43}} \\
		& \le \valu(\malloc_{r}) & \text{Observation \ref{graph-unchanged}} \\
		& \le \valu(\malloc'_{r}) & \\
		& = \virtualvalue_k(\malloc') & \text{Observation \ref{obs41}}.
	\end{align*}
	
	Now let $k = i$ and a good \(\good \in \malloc'_i\) and \(r = \roott{i}{\malloc'}\). We have:
	
	\begin{align*}
		\valu(\malloc'_i \setminus \{\good\}) & \le \valu(\malloc_i) & \text{\(\malloc'_i\) is minimal} \\
		& \le \valu(\malloc_{r}) & \text{$\rank_i(\malloc) = 1$} \\
		& \le \valu(\malloc'_{r}) & \\
		& = \virtualvalue_i(\malloc') & \text{Observation \ref{obs41}}.
	\end{align*}
	
	Therefore, \(\malloc'\) satisfies both Properties \ref{prop42} and \ref{prop43}.
	
	Since $\valu(\malloc_i) < \valu(\malloc'_i)$, and all other bundles remain unchanged, we have $\phi(\malloc) < \phi(\malloc')$. 
	
	In order to show that for every agent $k$ we have $\virtualvalue_k(\malloc) \le \virtualvalue_k(\malloc')$, let $r = \roott{k}{\malloc'}$. We have: 
	
	\begin{align*}
		\virtualvalue_k(\malloc) &\le \valu(\malloc_r) &\text{Observation \ref{graph-unchanged}} \\
		&\le \valu(\malloc'_r) & \\
		&= \virtualvalue_k(\malloc') &\text{Observation \ref{obs41}}.  
	\end{align*}
	
\end{proof}

\begin{proof}[of \cref{lem:U82}]
	During the update, only the bundle of agent $i$ is modified. \footnote{While other bundles may be transferred among agents, none is modified.} Therefore, Property \ref{prop42} remains valid for agents other than $i$. For agent $i$ we also know that $\malloc'_i \subseteq \relevant{\goods}{i, j}$. Therefore, Property \ref{prop42} holds for $\malloc'$. 
	
	To show that Property \ref{prop43} holds after the update, we note that this update rule is indeed exactly the same as Rule 1 in Section \ref{sec:eh}. Therefore, by Lemma \ref{virtual-value-increases} we conclude that virtual values do not decrease after the update. Furthermore, by Lemma \ref{no-virtual-se}, $\malloc'$ satisfies Property \ref{prop43}, and by Lemma \ref{nsw-increases} we have $\phi(\malloc) < \phi(\malloc')$. 
	
\end{proof}

\begin{proof}[of \cref{lem:U83}]
	According to Rule 3, for every remaining agent $j$, we have \( \valu_i(\malloc_j) = 0 \), meaning agent \( i \) isn't in agent \( j \)'s rankpath. Thus, \( \virtualvalue_j(\malloc) = \virtualvalue_j(\malloc') \).
	Also, the update keeps all the remaining agents' bundles unchanged. Thus, \( \malloc' \) satisfies Properties \ref{prop42} and \ref{prop43}.
	Finally, since $|\agents|$ decreases, we have \( \phi(\malloc) < \phi(\malloc') \).
	
\end{proof}

\begin{proof}[of \cref{no-se-1}]
	After the update, we have $\valu_i(\malloc'_0) \le \valu_i(\malloc^*_i)$, and for every remaining agent $j$, $\valu_i(\malloc'_j) = 0$. Therefore, $\valu_i(\cup \malloc') \le \valu_i(\malloc^*_i)$ which means that agent $i$ will not envy any remaining agent in subsequent steps.
	Furthermore, considering Property \ref{prop42} for $\malloc$, there exists an agent $j$ such that $\malloc_i \subseteq \relevant{\goods}{i, j}$. The only agent who might strongly envy $i$ is agent $j$. Post-update, $\malloc'_i$ can either be $\malloc_i$ or $\relevant{\malloc_0}{i}$.
	
	If $\malloc'_i = \malloc_i$, let $\good \in \malloc'_i$, and let $\malloc^*$ denote the final allocation. We have:
	
	\[
	\begin{aligned}
		\valu(\malloc'_i \setminus \{\good\}) &= \valu(\malloc_i \setminus \{\good\}) & \text{$\malloc'_i = \malloc_i$} \\
		&\le \virtualvalue_i(\malloc) & \text{Property \ref{prop43}} \\
		&\le \virtualvalue_j(\malloc) & \text{Observation \ref{path-virtual}} \\
		&\le \virtualvalue_j(\malloc^*) &  \\
		&\le \valu(\malloc^*_j).
	\end{aligned}
	\]
	
	Thus, agent $j$ does not strongly envy $i$ in the final allocation.
	
	Now, if $\malloc'_i = \relevant{\malloc_0}{i}$, for any remaining agent $j \in \agents'$ in the final allocation $\malloc^*$, we have:
	
	\[
	\begin{aligned}
		\valu_j(\malloc'_i) &= \valu(\relevant{\malloc_0}{i, j}) & \text{$\malloc'_i = \relevant{\malloc_0}{i}$} \\
		&\le \virtualvalue_j(\malloc) & \text{Rule 2 is not applicable} \\
		&\le \virtualvalue_j(\malloc^*) & \\
		&\le \valu(\malloc^*_j).
	\end{aligned}
	\]
	
	Therefore, agent $j$ does not strongly envy $i$ in the final allocation.
\end{proof}

\begin{proof}[of \cref{lem:cycle}]
	Since $\malloc$ satisfies Property \ref{prop42}, the in-degree of each vertex in $G_{0, \malloc}$ is equal to $1$. Additionally since Rule 3 is not applicable to $\malloc$, the out-degree of each vertex is at least $1$. Therefore $G_{0, \malloc}$ consists of one or more cycles. 
\end{proof}

\begin{proof}[of \cref{lem:U84}]
	First we show that the virtual value of each remaining agent does not decrease after the update. 	
	By Observation \ref{path-virtual} we have $\virtualvalue_i(\malloc) = \virtualvalue_{j_1}(\malloc) = \virtualvalue_{j_2}(\malloc) = \ldots = \virtualvalue_{j_k}(\malloc) = \valu(\malloc_i)$.
	Now let $r' = \roott{k}{\malloc'}$ and let $l$ be the agent such that $\malloc'_{r'} = \malloc_l$. For every remaining agent $j$ we have: 
	\begin{align*}
		\virtualvalue_j(\malloc) &= \virtualvalue_l(\malloc) & \\
		&\le \valu(\malloc_{l}) & \\
		&= \valu(\malloc'_{r'}) &\text{$\malloc'_{r'} = \malloc_l$} \\
		&= \virtualvalue_j(\malloc') &\text{$\roott{k}{\malloc'} = r'$}. 
	\end{align*}
	Hence, the virtual values of the remaining agents do not decrease.
	
	Since the set of bundles in $\malloc'$ remains unchanged, 	$\malloc'$ satisfies Property \ref{prop42}. 
	To Prove that $\malloc'$ satisfies Property \ref{prop43}, let $j$ be the remaining agent and $\good \in \malloc'_j$ and $\malloc'_j = \malloc_k$. We have: 
	
	\begin{align*}
		\valu(\malloc'_j \setminus \{\good\}) &= \valu(\malloc_k \setminus \{\good\}) &\text{$\malloc'_j = \malloc_k$} \\
		&\le \virtualvalue_k(\malloc) &\text{Property \ref{prop43}} \\
		&= \virtualvalue_j(\malloc) & \\
		&\le \virtualvalue_j(\malloc').
	\end{align*}
	
	Therefore $\malloc'$ satisfies both Properties \ref{prop42} and \ref{prop43}. 
	
	Since $|\agents'| = |\agents| - 1$, we have $\phi(\malloc) < \phi(\malloc')$. 
\end{proof}

\begin{proof}[of \cref{no-se-2}]
	Since only $\malloc_0, \malloc_i, \malloc_{j_1}$ may be relevant to agent $i$, and this agent picks the more valuable bundle between $\malloc_i \cup \relevant{\malloc_0}{i}$ and $\malloc_{j_1}$, it doesn't matter what happens in the future, and $i$ will not envy any bundle in $\malloc^*$. 
	
	Suppose that $j$ is the corresponding agent of agent $i$. 
	There are two cases for $\malloc^*_i$. 
	The first case is $\malloc'_i = \malloc_i \cup  \relevant{\malloc_0}{i}$. In this case for agent $k \neq j$ we have: 
	
	\begin{align*}
		\valu_k(\malloc^*_i) &= \relevant{\malloc_0}{i, k}& \text{$\malloc_i \subseteq \relevant{\goods}{i, j}$} \\
		&\le \virtualvalue_k(\malloc) &\text{Rule 2 is not applicable} \\
		&\le \virtualvalue_k(\malloc^*) & \\
		&\le \valu_k(\malloc_k^*). 
	\end{align*}
	
	and for agent $j$ we have: 
	
	\begin{align*}
		\valu_j(\malloc^*_i) &= \valu(\relevant{\malloc_i}{i, j}) &\text{Rule 1 is not applicable} \\
		&= \valu(\malloc_i) &\text{$\malloc_i \subseteq \relevant{\goods}{i, j}$} \\
		&= \virtualvalue_j(\malloc) &\text{Observation \ref{obs41}} \\
		&\le \virtualvalue_j(\malloc^*) & \\
		&\le \valu_j(\malloc_j^*). 
	\end{align*}
	
	The second case is $\malloc'_i = \malloc_{j_1}$. In this case only $j_1$ may envy $i$. Let $\good \in \malloc_{j_1}$. We have: 
	
	\begin{align*}
		\valu(\malloc^*_i \setminus \{\good\}) &= \valu(\malloc_{j_1} \setminus \{\good\}) &\text{$\malloc^*_i = \malloc_{j_1}$} \\
		&\le \virtualvalue_{j_1}(\malloc) &\text{Property \ref{prop43}}
		\\
		&\le \virtualvalue_{j_1}(\malloc^*) &\\
		&\le \valu_{j_1}(\malloc_{j_1}^*). 
	\end{align*}
	
	Therefore no agent in $\malloc^*$ will strongly envy $i$.  
\end{proof}

\begin{proof}[of \cref{thm8}]
	In this algorithm, we satisfy all agents one by one. By Lemmas \ref{no-se-1} and \ref{no-se-2}, the returned allocation by $\algopr$ is $\efx$. 
\end{proof}

==> src/appcase1.tex <==
\section{Missing Proofs \ref{sec:5}}

\begin{proof}[of \cref{lem:511}]
	The only agent whose value for her bundle is changed is agent $i$, and the allocated good $\good$ is relevant to agent $i$. Therefore, Property \ref{prop:2} holds. Furthermore, $\valu(\malloc'_i) > \valu(\malloc_i)$ and  by Lemma \ref{lem:phi} we have $\phi(\malloc) < \phi(\malloc')$. 
\end{proof}

\begin{proof}[of \cref{lem:521}]
	Given that agent 
	$i$
	selects only relevant goods from the pool, we have $\valu_i(\malloc'_i) = \valu({\malloc'_i})$. Furthermore, according to Lemma \ref{lem:12}, for every edge $i_1 \rightarrow i_2$ in the path from $j$ to $i$, we have  $\valu_{i_1}(\malloc'_{i_2}) = \valu(\malloc'_{i_2})$. Consequently, Property \ref{prop:2} remains valid after the update.
	To prove $\phi(\malloc) < \phi(\malloc')$, we utilize Lemma \ref{lem:phi}. Considering $A,x,x'$ in the statement of Lemma \ref{lem:phi} we proceed with: 
	\begin{align*}
		A &= \mbox{Agents in the path from $j$ to $i$ } \\
		x &= \min_{i' \in A}(\valu(\alloc_{i'})) = \valu(\malloc_j) \\
		x' &= \min_{i' \in A}(\valu(\alloc'_{i'}))
	\end{align*}
	Also, since for agent $i$, $\valu(\malloc_j) < \invsq\valu(\malloc_i) 
	< \valu(\malloc'_i),
	$
	and for every other agent $k \in A$, $\valu(\malloc_j) < \invsq\valu(\malloc_{k})$, we have $x < x'$.  
	Finally, agent $j$ is a source in $G_{\sqrt{2}, \malloc}$ and therefore, $x = \valu(\malloc_j)$. Thus, all conditions of Lemma \ref{lem:phi} are satisfied, which implies $\phi(\malloc) < \phi(\malloc')$.
\end{proof}

\begin{proof}[of \cref{thm:fstep}]
	Let $\malloc$ be the allocation before the final step.
	First, note that agent $1$ is a source in $G_{\sqrt{2}, \malloc}$. We prove that after this allocation, no-one will $\sqrt{2}$-envy $\malloc^*_1$. As a contradiction, 
	suppose agent $i$ $\sqrt{2}$-envies agent $1$. Since agent $1$ was a source, agent $i$ did not $\sqrt{2}$-envy him before the final step. This means that the pool has a non-zero value for agent $i$, and given the fact that Rule 1 was not applicable, agent $i$ is not a source. Now, suppose that agent $j$ is a source that has a path to $i$. We have
	\begin{align*}
		\valu_i(\malloc^*_1) &= \valu(\malloc_1) + \valu_i(\malloc_0) \\
		&\leq  \valu(\malloc_j) + \valu_i(\malloc_0) &\valu(\malloc_1) \leq\valu(\malloc_j)  \\
		&\leq \frac{\sqrt{2}}{2}\valu(\malloc_i)  + \valu_i(\malloc_0) & \mbox{ $j$  has a path to $i$ in }G_{\sqrt{2},\malloc}\\
		&\leq \frac{\sqrt{2}}{2}\valu(\malloc_i)  + \frac{\sqrt{2}}{2}\valu(\malloc_i) & \mbox{$i$ does not $\sqrt{2}$-envy $\malloc_0$}\\
		&\leq \sqrt{2}\valu(\malloc_i). 
	\end{align*}
	But this contradicts the fact that agent $i$ does not $\sqrt{2}$-envy agent $j$ before the final step.
\end{proof} 

==> src/appcase1tex.tex <==
\section{Missing Proofs \ref{sec:5}}

\begin{proof}[of \cref{lem:511}]
	The only agent whose value for her bundle is changed is agent $i$, and the allocated good $\good$ is relevant to agent $i$. Therefore, Property \ref{prop:2} holds. Furthermore, $\valu(\malloc'_i) > \valu(\malloc_i)$ and  by Lemma \ref{lem:phi} we have $\phi(\malloc) < \phi(\malloc')$. 
\end{proof}

\begin{proof}[of \cref{lem:521}]
	Given that agent 
	$i$
	selects only relevant goods from the pool, we have $\valu_i(\malloc'_i) = \valu({\malloc'_i})$. Furthermore, according to Lemma \ref{lem:12}, for every edge $i_1 \rightarrow i_2$ in the path from $j$ to $i$, we have  $\valu_{i_1}(\malloc'_{i_2}) = \valu(\malloc'_{i_2})$. Consequently, Property \ref{prop:2} remains valid after the update.
	To prove $\phi(\malloc) < \phi(\malloc')$, we utilize Lemma \ref{lem:phi}. Considering $A,x,x'$ in the statement of Lemma \ref{lem:phi} we proceed with: 
	\begin{align*}
		A &= \mbox{Agents in the path from $j$ to $i$ } \\
		x &= \min_{i' \in A}(\valu(\alloc_{i'})) = \valu(\malloc_j) \\
		x' &= \min_{i' \in A}(\valu(\alloc'_{i'}))
	\end{align*}
	Also, since for agent $i$, $\valu(\malloc_j) < \invsq\valu(\malloc_i) 
	< \valu(\malloc'_i),
	$
	and for every other agent $k \in A$, $\valu(\malloc_j) < \invsq\valu(\malloc_{k})$, we have $x < x'$.  
	Finally, agent $j$ is a source in $G_{\sqrt{2}, \malloc}$ and therefore, $x = \valu(\malloc_j)$. Thus, all conditions of Lemma \ref{lem:phi} are satisfied, which implies $\phi(\malloc) < \phi(\malloc')$.
\end{proof}

\begin{proof}[of \cref{thm:fstep}]
	Let $\malloc$ be the allocation before the final step.
	First, note that agent $1$ is a source in $G_{\sqrt{2}, \malloc}$. We prove that after this allocation, no-one will $\sqrt{2}$-envy $\malloc^*_1$. As a contradiction, 
	suppose agent $i$ $\sqrt{2}$-envies agent $1$. Since agent $1$ was a source, agent $i$ did not $\sqrt{2}$-envy him before the final step. This means that the pool has a non-zero value for agent $i$, and given the fact that Rule 1 was not applicable, agent $i$ is not a source. Now, suppose that agent $j$ is a source that has a path to $i$. We have
	\begin{align*}
		\valu_i(\malloc^*_1) &= \valu(\malloc_1) + \valu_i(\malloc_0) \\
		&\leq  \valu(\malloc_j) + \valu_i(\malloc_0) &\valu(\malloc_1) \leq\valu(\malloc_j)  \\
		&\leq \frac{\sqrt{2}}{2}\valu(\malloc_i)  + \valu_i(\malloc_0) & \mbox{ $j$  has a path to $i$ in }G_{\sqrt{2},\malloc}\\
		&\leq \frac{\sqrt{2}}{2}\valu(\malloc_i)  + \frac{\sqrt{2}}{2}\valu(\malloc_i) & \mbox{$i$ does not $\sqrt{2}$-envy $\malloc_0$}\\
		&\leq \sqrt{2}\valu(\malloc_i). 
	\end{align*}
	But this contradicts the fact that agent $i$ does not $\sqrt{2}$-envy agent $j$ before the final step.
\end{proof} 

==> src/applexico.tex <==
\section{Missing Proofs}
 Lemma \ref{lem:phi} helps us prove some of our claims in Section \ref{sec:5}. A Lemma similar to Lemma \ref{lem:phi} has been previously proved by Akrami \etal.\cite{akrami2022ef2x}. For completeness, here we restate and prove this lemma.
 \begin{lemma}\label{lem:phi}
Let $\alloc$ and $\alloc'$ be two allocations. Define:
 	\begin{align*}
 		A = \{i | \alloc_i \neq \alloc'_i\} \\
 		x = \min_{i \in A}(\valu(\alloc_i)) \\
 		x' = \min_{i \in A}(\valu(\alloc'_i)).
 	\end{align*}
 Assume the following conditions hold:
 \begin{itemize}
 	\item $x < x'$,
 	\item There is only one source agent in $A$ in $G{\beta,\alloc}$,
 	\item If $i$ is the source agent in $A$, then $\valu(\alloc_i)=x$.
 \end{itemize}
 Then, $\phi(\alloc) < \phi(\alloc')$.
 \end{lemma}
  \begin{proof}
  	 Denote the sources of $G_{\beta, \alloc}$ by $s_1, s_2, \ldots, s_k$ and the sources of $G_{\beta, \alloc'}$ by $s'_1, s'_2, \ldots, s'_{k'}$. Then:
 	\begin{align*}
	\phi(\alloc) = \big[ \valu(\alloc_{s_1}),\valu(\alloc_{s_2}),\ldots, \valu(\alloc_{s_k}),\infty \big], \\
	\phi(\alloc') = \big[ \valu(\alloc'_{s'_1}),\valu(\alloc'_{s'_2}),\ldots, \valu(\alloc'_{s'_{k'}}),\infty \big].
\end{align*}
 	Since agent $i$ is a source in $G_{\beta, \alloc}$, we can assume without loss of generality that there exist an index $l$ such that $s_l = i$, and $\valu(\alloc_{s_l}) \neq \valu(\alloc{s_{l+1}})$. (we can reorder same values in $\phi$ to satisfy this condition). We show that for every $l' < l$ we have $\phi(\alloc)_{l'} = \phi(\alloc')_{l'}$ and for $l$ we have $\phi(\alloc)_l < \phi(\alloc')_l$. 
 	\begin{itemize}
 		\item For every $l' < l$, we claim that $s_{l'}$ remains a source in $G_{\beta, \alloc'}$. To prove this, we show that for every agent $j$ we have $\valu_j(\alloc'_{s_{l'}}) < \beta \valu_j(\alloc'_j)$. If $j \notin A$, our claimi is trivial since $s_{l'}$ is a source in $G_{\beta, \alloc}$. If $j \in A$, we have: 
 		\begin{align*}
 			\valu_j(\alloc'_{s_{l'}}) &\le \valu(\alloc'_{s_{l'}}) &\\
 			&= \valu(\alloc_{s_{l'}}) &\text{$s_{l'} \notin A$}\\
 			&\le x &\text{$l' < l$}, \\
 			&< x' \\
 			&\le \valu(\alloc'_j) &\text{$j \in A$},\\
 			&= \valu_j(\alloc'_j) &\\
 			&\le \beta \valu_j(\alloc'_j). 
 		\end{align*}
 		Therefore $j$ does not $\beta$-envy $s_{l'}$ in $\alloc'$ and $\phi(\alloc)_{l'} = \phi(\alloc')_{l'}$. 
 		
 		\item To prove $\phi(\alloc)_l < \phi(\alloc')_l$, we need to show that for any source agent $j$ in $G_{\beta, \alloc'}$ 
 		such that $j \notin \{s_1, s_2, \dots, s_{l - 1}\}$ we have $\valu(\alloc'_j) > x = \phi(\alloc)_l$. 
 		We have three cases. 
 		The first case is $j \in A$. In this case we have: 
 		\begin{align*}
 			\phi(\alloc)_l &= x &\\
 			& < x'\\
 			&\le \valu(\alloc'_j) &\text{$j \in A$}. 
 		\end{align*}
 		In the second case we have $j \notin A$ and $j$ is also a source in $G_{\beta, \alloc}$. In this case we have: 
 		\begin{align*}
 			\phi(\alloc)_l &= x &\\
 			&< \valu(\alloc_j) &\text{$j \notin {s_1, s_2, \dots, s_{l - 1}}$},\\
 			&= \valu(\alloc'_j) &\text{$j \notin A$}. 
 		\end{align*}
 		In the last case we have $j \notin A$ and $j$ is not a source in $G_{\beta, \alloc}$. We know there exists another agent $j' \in A$ such that $j'$ $\beta$-envies agent $j$ in $G_{\beta, \alloc}$. Therefore we have: 
 		\begin{align*}
 			\phi(\alloc)_l &= x &\\
 			&< \sqrt{2} x &\\
 			& \le\sqrt{2} \valu(\alloc_{j'}) &\text{$j' \in A$},\\
 			&< \valu(\alloc_j) &\text{$j'$ envies $j$ in $\alloc$},\\
 			&= \valu(\alloc'_j) &\text{$j \notin A$}. 
 		\end{align*}
 	\end{itemize}
 	Hence, $\phi(\alloc')_l$ is replaced with an agent with a larger value, or $\phi(\alloc')_l = \infty$. 
 	
 \end{proof}.


==> src/case3/U1.tex <==
\subsection{Update Rule 1}
The purpose of this rule is to remove envy cycles in $G_{1, \malloc}$. When there is an envy cycle $\cycle$ in $G_{1, \malloc}$, we proceed by transferring bundles along the cycle. That is, for each edge $i \rightarrow j \in \cycle$, we set $\malloc'_i = \relevant_i(\malloc_j)$. Additionally for every agent $i \notin \cycle$, we set $\malloc'_i = \relevant_i(\malloc_i)$. 

\iffalse
\vspace{0.1cm}
\begin{tcolorbox}[colback=white!5,coltitle=white!95!black,colframe=black!95,
	title= \textbf{Update Rule $1$}]
	
	\textbf{Preconditions:}
	\begin{itemize}
		\item $\malloc$ satisfies Property \ref{prop:51}. 
		\item There exists a cycle $i_1 \rightarrow i_2 \rightarrow \ldots \rightarrow i_k \rightarrow i_1$ in $G_{1,\malloc}$. 
	\end{itemize}
	
	\textbf{Update:}
	\begin{itemize}
		\item $\malloc'_j = \begin{cases}
			\relevant_j(\malloc_j) & j \in [n] \setminus \{i_1,i_2,\ldots,i_k\}\\
			\relevant_{i_l}(\malloc_{i_{l\%k+1}}) & j = i_l \mbox{ for } 1 \le l \le k
		\end{cases}$
	\end{itemize}
\end{tcolorbox}
\fi

\begin{lemma}\label{lem:711}
	Let $\malloc'$ be the allocation after Rule 1. Then $\malloc'$ is $\efx$ and satisfies Property \ref{prop:51}.
\end{lemma}
\begin{proof}
	After applying Rule 1, for every agent $i$, we have $\valu_i(\malloc'_i) \ge \valu_i(\malloc_i)$. Furthermore, each bundle in $\malloc'$ is a subset of a bundle in $\malloc$.  Therefore  since $\malloc$ had no strongly envy, $\malloc'$ also has no strongly envy.
	
	For agents not involved in the cycle, we have $\malloc'_i = \relevant_i(\malloc_i)$. As per the definition, all goods in $\relevant_i(\malloc_i)$ are relevant to agent $i$. Also, for every edge $i \rightarrow j \in \cycle$ we have $\malloc'_i = \relevant_i(\malloc'_j)$.  By definition, all goods in $\malloc'_i$ are relevant to agent $i$. Therefore,  Property \ref{prop:51} holds.
\end{proof}

\begin{lemma}\label{lem:712}
	Let $\malloc'$ be the allocation after applying Rule 1. We have $\phi(\malloc') > \phi(\malloc)$. 
\end{lemma}
\begin{proof}
	For every agent $i$ we have $\valu_i(\malloc'_i) \ge \valu_i(\malloc_i)$. Furthermore for every agent $i \in \cycle$, we have $\valu_i(\malloc'_i) > \valu_i(\malloc_i)$. Thus we have:
	\begin{align*}
		\sum_{i=1}^{n} \valu_i(\malloc'_i) > \sum_{i=1}^{n} \valu_i(\malloc_i).
	\end{align*}
	Therefore $\phi(\malloc') > \phi(\malloc)$.
\end{proof}

==> src/case4/phase1-intro.tex <==
\subsection{Phase 1}
In the first phase, we use two updating rules to update the allocation. We ensure that after each update, our allocation satisfies the following two properties:

\begin{enumerate}[label=\textcolor{red}{$\uparrow\!\!$} (\roman*)]
	\item \label{same-type}
	For every agent $i$ there exist an agent $j$ such that $\malloc_i \subseteq \relevant{\goods}{i, j}$,
	\item \label{efx-father}
	For every agent $i$ and every good $\good \in \malloc_i$ we have $\valu(\malloc_i \setminus \{\good\}) \le \valufather$.
\end{enumerate}
Note that if $\malloc(i) \subseteq \relevant{\goods}{i,j}$, the agent $j$ is the only agent that might envy agent $i$. Moreover, for every $k \neq i,j$, we have $\valu_k(\malloc_i)=0$. Furthermore, we have $\valu_i(\malloc_i) = \valu_j(\malloc_i) = \valu(\malloc_i)$. 
We use the social welfare as the potential function to prove the termination of Phase 1:
\begin{align*}
	\phi(\malloc) = \sum_{i = 1}^{n} \valu(\malloc_i).
\end{align*}

Before introducing our updating rules, we outline some key observations and lemmas that are essential for analyzing our allocation algorithm.





 
%\begin{observation} \label{obs-all-relevant}
%	Let $\malloc$ be an allocation that satisfies Property \ref{same-type}. Then, all the goods in $\malloc_i$ are relevant to agent $i$.
%\end{observation}

%\begin{observation} \label{obs-more-than-father}
%	Let $\malloc$ be an allocation that satisfies Property \ref{same-type}. Then for every agent $i$, we have $\valu(\malloc_i) \ge \valufather$.
%\end{observation}

%\begin{lemma} \label{lem-p2-deg1}
%	Let $\malloc$ be an allocation that satisfies Property \ref{same-type}. Then every agent $i$ has at most one incoming edge in $\ptgraph$.
%\end{lemma}
%\begin{proof}
%	Since allocation $\malloc$ satisfies Property \ref{same-type}, there exist a not necessarily different agent $j$ such that $\malloc_i \subseteq \edge_{i, j}$. Furthermore, for any other agent $k$ that $k \ne i$ and $k \ne j$ we have $\valu_k(\malloc_i) = 0$. This is because all the goods in $\edge_{i, j}$ are irrelevant to agent $k$. Therefore, the only possible incoming edge for agent $i$ is from agent $j$, and agent $i$ can have at most one incoming edge.
%\end{proof}

%\begin{lemma} \label{incoming-edge-relevant}
%	Let $\malloc$ be an allocation satisfying Property \ref{same-type}. Then for every agent $i$ and $j$ such that there exist an edge from $j$ to $i$ in $\ptgraph$, we have $\valu_j(\malloc_i) = \valu(\malloc_i)$.
%\end{lemma}
%\begin{proof}
%	By the definition of $\ptgraph$ there exist a good $\good \in \malloc_i$ that is relevant to agent $j$. Furthermore  since good $\good$ is relevant to both agents $i$ and $j$, we have $\good \in \edge_{i, j}$. Since $\malloc$ satisfies Property \ref{same-type} it follows that $\malloc_i \subseteq \edge_{i, j}$ and all the goods in $\malloc_i$ are also relevant to agent $j$. Therefore we have $\valu_j(\malloc_i) = \valu(\malloc_i)$.
%\end{proof}


%\begin{lemma} \label{same-father}
%	Let $\malloc$ be an allocation that satisfies Property \ref{same-type}. Let $i$ and $j$ be two agents such that there exists an edge from agent $j$ to agent $i$ in $\ptgraph$. Then, $\father_{\malloc, i} \in \{i,\father_{\malloc, j}\}$.
%\end{lemma}
%\begin{proof}
%	By Lemma \ref{lem-p2-deg1} we know that agent $j$ is the only agent with an outgoing   edge to agent $i$. Hence, the set of vertices that can reach agent $i$ includes agent $i$ itself and all vertices that can reach agent $j$. This immediately implies Lemma \ref{same-father}.
%\end{proof}

%\begin{observation} \label{path-father}
%	Consider an allocation $\malloc$ that satisfies Property \ref{same-type}. For any agents $i$ and $j$ such that $j$ appears in the path from agent $\father_{\malloc, i}$ to agent $i$ in $\ptgraph$, it can be observed that $\father_{\malloc, i} = \father_{\malloc, j}$.
%\end{observation}


%\begin{lemma} \label{less-father}
%	Let $\malloc$ be an allocation that satisfies Property \ref{same-type}. Let $i$ and $j$ be two agents such that there exists an edge from agent $j$ to agent $i$ in $\ptgraph$. Then, $\vfather{\malloc}{\malloc}{i} \le \vfather{\malloc}{\malloc}{j}$
%\end{lemma}
%\begin{proof}
%	By definition \ref{father-def}, there exist a path from agent $\father_{\malloc, j}$ to agent $j$ in $\ptgraph$. Furthermore since there is an edge from agent $j$ to agent $i$, $\father_{\malloc, j}$ also has a path to agent $i$. Therefore $\valu(\father_{\malloc, i}) \le \valu(\father_{\malloc, j})$.
%\end{proof}

\begin{lemma}\label{Caaw}
Consider an allocation $\malloc$ satisfying both Properties \ref{same-type} and \ref{efx-father}. Then, $\malloc$ is $\efx$.
\end{lemma}
\begin{proof}
Suppose that some agent $j$ envies agent $i$. We show that this envy is not strong. By Property \ref{same-type}, we know $\malloc_i \in \relevant{\goods}{i,j}$. Furthermore, since agent $j$ is the only agent that envies agent $i$, we have $\father_{\malloc, i} = \father_{\malloc, j}$.

Therefore, we have:
	
%	If no agent envies another agent, then the $\efx$ property is trivial. Therefore, assume that there exists two agent $i$ and $j$ such that agent $j$ envies agent $i$, which implies that there is an edge from $j$ to $i$ in $\ptgraph$. By Property \ref{same-type}, we know that $j$ is the only agent with outgoing edge to $i$. Furthermore, we have $\valu(\malloc_j) < \valu(\malloc_i)$, which means $\father_{\malloc, i} \ne i$. According to Lemma \ref{same-father}, it follows that $\father_{\malloc, i} = \father_{\malloc, j}$ Therefore for every good $\good \in \malloc_i$ we have:
	\begin{align*}
		\valu_j(\malloc_i \setminus \{g\}) &= \valu(\malloc_i \setminus \{g\}) & \mbox{ Property \ref{same-type}} \\
		&\le \valufather  & \mbox{ Property \ref{efx-father}}\\
		&= \valu(\malloc_{\father_{\malloc, j}}) & \father_{\malloc, i} = \father_{\malloc, j}\\
		& \le \valu(\malloc_j) & \eqref{fless} \\
		& = \valu_j(\malloc_j).  
	\end{align*}
	Therefore, agent $j$ does not strongly envy agent $i$, and the proof is complete.
\end{proof}



==> src/case4/phase1-u1.tex <==
\subsubsection*{Update Rule 1}
This updating rule is feasible when there exists  an agents $i$ and $j$ ($i$ can be the same agent as $j$) such that $\father_{\malloc, i} = i$ and $\malloc_i$ is a non-empty subset of $\relevant{\goods}{i, j}$, and there exists at least one good $\good \in \relevant{\malloc_{0}}{i, j}$. 
We set $\malloc'_i$ to a minimal subset of $\malloc_i \cup \{\good\}$ such that $\valu(\malloc'_i) > \valu(\malloc_i)$.


\begin{lemma}\label{prop:81}
	After applying Rule 1, $\malloc'$ satisfies properties \ref{same-type} and \ref{efx-father}. 
\end{lemma}
\begin{proof}
	Since $\malloc_i$ and  $\good$ belong to $\relevant{\goods}{i,j}$, Property \ref{same-type} holds. To prove Property \ref{efx-father}, we only need to verify it for agent $i$. Since $\malloc'_i$ is a minimal subset of $\malloc_i \cup \{\good\}$ such that $\valu(\malloc'_i) >\valu(\malloc_i)$, for every good $\good' \in \malloc'_i$ we have $\valu(\malloc'_i \setminus \{\good'\}) \leq \valu(\malloc_i)$. Furthermore, we have $\valu(\malloc_i) = \valu(\father_{\malloc, i}) \leq \valu(\father_{\malloc', i}), $ which means Property \ref{efx-father} satisfies for agent $i$. 
\end{proof}
\begin{lemma}\label{termination}
	After applying Update Rule 1, we have $\phi(\malloc') > \phi(\malloc)$
\end{lemma}
\begin{proof}
	Since bundle of agent $i$ is the only modified bundle and $\valu(\malloc_i) < \valu(\malloc'_i)$, we have $
		\phi(\malloc')> \phi(\malloc)$.
\end{proof}


==> src/case4/phase1-u2.tex <==
\subsubsection*{Update Rule 2}
The second update rule applies when there are two (not necessarily distinct) agents $i$ and $j$, such that $\valu(\relevant{\malloc_{0}}{i, j}) > \valufather$ and $\valufather \le \vfather{\malloc}{\malloc}{j}$. Let $P$ be the path from  $\father_{\malloc, i}$ to $i$. We transfer the bundles through this path, that is, for every edge $k \rightarrow l \in P$ we allocate $\malloc_l$ to $k$. Also, we set 
$\malloc'_i$ to a minimal subset of $\relevant{\malloc_0}{i, j}$ with value more than $\valufather$, and furthermore, return 
$\malloc_{\father_{\malloc, i}}$ back to the pool. 

%Before we prove the main properties of Rule 2, let us fix some notations.
% We define $\ptagentset$ as the set of agents $k$ such that $\father_{\malloc, k} = \father_{\malloc, i}$. Additionally, we define $\ptpath$ as the path from agent $\father_{\malloc, i}$ to agent $i$ in $\ptgraph$. Agents in the path are represented by $\ptpathagents_1, \ptpathagents_2, \dots, \ptpathagents_l$, in the order of appearance in the path. Note that $\ptpathagents_1 = \father_{\malloc, i}$ and $\ptpathagents_l = i$, and there exists an edge from $\ptpathagents_k$ to $\ptpathagents_{k+1}$ in $\ptgraph$ for every $1\leq k < l$.

%\begin{lemma} \label{p2-path-same-father}
%	For every $k \in \ptpath$ we have $\father_{\malloc, k} = \father_{\malloc, i}$.
%\end{lemma}
%\begin{proof}
%	According to Lemma \ref{same-father}, it follows that for any edge $k' \rightarrow k \in \ptgraph$, $\father_{\malloc, k}$ equals $\father_{\malloc, k'}$. Consequently, for any agent $k \in \ptpath$, $\father_{\malloc, k}$ is equal to $\father_{\malloc, i}$.
%\end{proof}

%\begin{lemma} \label{p2-path-reverse}
%	After applying  Rule 2, for each $1 \le k < l$, there exists an edge from agent $\ptpathagents_{k + 1}$ to agent $\ptpathagents_k$ in $\nptgraph$. This modification results in a reversal of the edge direction along the path $\ptpath$.
%\end{lemma}
%\begin{proof}
%	For every $1 \le k < l$, we have that $\malloc'_{\ptpathagents_{k}} = \malloc_{\ptpathagents_{k + 1}}$. Additionally, by Lemma \ref{incoming-edge-relevant}, the goods in $\malloc_{\ptpathagents_{k + 1}}$ are relevant to both agents $\ptpathagents_k$ and $\ptpathagents_{k + 1}$. Therefore, after applying Rule 2, the goods present in $\malloc'_{\ptpathagents_{k}}$ are relevant to agent $\ptpathagents_{k + 1}$, and there is an edge from agent $\ptpathagents_{k + 1}$ to agent $\ptpathagents_k$ in $\nptgraph$. Furthermore, by Lemma \ref{lem-p2-deg1}, agent $\ptpathagents_{k + 1}$ is the only incoming edge of agent $\ptpathagents_{k}$. This completes the proof.
%\end{proof}

%\noindent
%\textbf{Differences of graphs $\ptgraph$ and $\nptgraph$:}
%The only bundles that have been modified are the bundles of the agents in $\ptpath$. As a result, only the incoming edges of the vertices in $\ptpath$ have been changed. Based on Lemma \ref{p2-path-reverse}, the edges in $\ptpath$ have been reversed in direction. Additionally, if $i \ne j$, the goods in the new bundle of agent $i$ are relevant to agent $j$, and an edge has been added to the graph from agent $j$ to agent $i$. Note that, by Lemma \ref{lem-p2-deg1}, each vertex has a maximum of one incoming edge,  and agents in $\ptpath$ do not have any other incoming edges.

\begin{lemma} \label{p2-phase1-u2-vk-ge-vfather}
	For every agent $k$ we have $\valu(\malloc'_k) \ge \vfather{\malloc}{\malloc}{k}$.
\end{lemma}
\begin{proof}
	If $k \notin \ptpath$, the statement is trivial since the bundle of agent $k$ has not changed and $\valu(\malloc'_k) = \valu(\malloc_k) \ge \vfather{\malloc}{\malloc}{k}$. If $k \in \ptpath$ and $k \ne i$, let $l$ be the agent such that $k \rightarrow l \in P$. We have $\father_{\malloc, k} = \father_{\malloc, l} = \father_{\malloc, i}$. Additionally, we have $\malloc'_k = \malloc_{l}$. Therefore,
	\begin{align*}
		\valu(\malloc'_k) &= \valu(\malloc_{l}) \\
		&\ge \vfather{\malloc}{\malloc}{l}  \\
		&= \vfather{\malloc}{\malloc}{k}. 
	\end{align*}
	Moreover, for agent $i$, $\malloc'_i$ is a minimal subset of $\relevant{\malloc_0}{i, j}$ satisfying $\valu(\malloc'_i) > \valufather$. Therefore, the statement also holds for agent $i$. This completes the proof.
\end{proof}

\begin{lemma} \label{p2-phase1-u2-vk-le-vkp}
%	\alireza{TODO: replace $k$ and $k'$ everywhere}
	For each edge $k \rightarrow l \in \nptgraph$, we have $\vfather{\malloc}{\malloc}{k} \ge \vfather{\malloc}{\malloc}{l
	}$. %Note that this condition considers the agent's allocation and father before applying the update rule, but uses the graph after applying the update rule.
\end{lemma}
\begin{proof}
	We distinguish between three cases:
	\begin{itemize}
		\item \textbf{Case 1: $k \notin \ptpath$} Since the bundle of agent $k$ remains unchanged, the incoming edges of agent $k$ also remain the same. Hence $k \rightarrow l \in \nptgraph$ and therefore we have $\vfather{\malloc}{\malloc}{k} \ge \vfather{\malloc}{\malloc}{l}$.
		\item \textbf{Case 2: $k,l \in \ptpath$.} We have $\father_{\malloc, k} = \father_{\malloc, l}$ which immediately implies $\vfather{\malloc}{\malloc}{k} \ge \vfather{\malloc}{\malloc}{l}$.
		\item  \textbf{Case 3: $l \notin \ptpath, k \in \ptpath$.} This case only happens when $l = j$ and $k = i$, which by  precondition of Rule 2, we have $\valufather \le \vfather{\malloc}{\malloc}{j}$.
	\end{itemize}
\end{proof}

\begin{lemma} \label{p2-phase1-u2-induction}
	For every agent $k$ we have $\vfather{\malloc}{\malloc}{k} \le \vfather{\malloc'}{\malloc'}{k}$.
\end{lemma}
\begin{proof}
	Let $d$ be the length of the path 
	from $\father_{\malloc', k}$ to $k$ in $\nptgraph$.
	We use induction on $d$. For the base case, if $d=0$, we know $\father_{\malloc', k} = k$. Hence we have:
	\begin{align*}
		\vfather{\malloc'}{\malloc'}{k} &= \valu(\malloc'_k) & \mbox{ $\father_{\malloc', k} = k$} \\
		&\ge \vfather{\malloc}{\malloc}{k}  & \mbox{ Lemma \ref{p2-phase1-u2-vk-ge-vfather}}.
	\end{align*}
	Now suppose the statement holds for every $d' < d$. Our goal is to prove the claim for $d$.  Let $l$ be the agent that precedes $k$ in the path from $\father_{\malloc', k}$. Since $\father_{\malloc', k} = \father_{\malloc', l}$, we have:
	\begin{align*}
		\vfather{\malloc'}{\malloc'}{k} &= \vfather{\malloc'}{\malloc'}{l} & \mbox{ $\father_{\malloc', k} = \father_{\malloc', l}$} \\
		&\ge \vfather{\malloc}{\malloc}{l}  & \mbox{ induction hypothesis}\\
		&\ge \vfather{\malloc}{\malloc}{k} & \mbox{ Lemma \ref{p2-phase1-u2-vk-le-vkp}}.
	\end{align*}
\end{proof}

\begin{lemma}\label{pl:1}
	After applying Rule 2, $\malloc'$ satisfies properties \ref{same-type} and \ref{efx-father}. 
\end{lemma}
\begin{proof}
	We prove each property separately.
	To show Property \ref{same-type}, note that for every vertex $j \notin P$, we have $\malloc_k = \malloc'_k$. So given that Property \ref{same-type} holds for agent $k$ before the update, it also holds thereafter. Furthermore, for every edge $k \rightarrow l \in P$, we have $\malloc'_k = \malloc_{l}$.  By Property \ref{same-type} for $\malloc$ we know $\malloc'_k = \malloc_{l} = \relevant{\goods}{k,l}$. Also, for agent $i$ we know $\malloc'_{i} \in \relevant{\malloc_{0}}{i,j}$. Therefore, Property \ref{same-type} holds for $\malloc'$.
	
	To prove Property \ref{efx-father} we consider three cases.
	\begin{itemize}
		\item \textbf{Case 1: $k \notin \ptpath$.} The bundle of agent $k$ remains unchanged. Therefore for every good $\good \in \malloc'_k$ we have:
		\begin{align*}
			\valu(\malloc'_k \setminus \{\good\}) &= \valu(\malloc_k \setminus \{\good\}) & \mbox{$\malloc'_k = \malloc_k$} \\
			&\le \vfather{\malloc}{\malloc}{k}  & \mbox{$\malloc$ satisfies Property \ref{efx-father}}\\
			&\le \vfather{\malloc'}{\malloc'}{k}. & \mbox{Lemma \ref{p2-phase1-u2-induction}}
		\end{align*}
		\item \textbf{Case 2: $k \in \ptpath$ and $k \ne i$.} 
		There exist an agent $l \in \ptpath$ such that $\malloc'_k = \malloc_{l}$. Hence for every good $\good \in \malloc'_k$ we have: 
		\begin{align*}
			\valu(\malloc'_k \setminus \{\good\}) &= \valu(\malloc_{l} \setminus \{\good\}) & \mbox{$\malloc'_k = \malloc_{l}$} \\
			&\le \vfather{\malloc}{\malloc}{l}  & \mbox{$\malloc$ satisfies Property \ref{efx-father}}\\
			&= \vfather{\malloc}{\malloc}{k}  & \mbox{ $\father_{\malloc, k} = \father_{\malloc, l}$}\\
			&\le \vfather{\malloc'}{\malloc'}{k}. & \mbox{Lemma \ref{p2-phase1-u2-induction}}
		\end{align*}
		\item  \textbf{Case 3: $k = i$} By the way we perform Rule 2, $\malloc'_i$ is the minimal subset of $\malloc_0 \cap \relevant{\malloc_{0}}{i, j}$ with value more than $ \valufather$. Thus, for every good $\good \in \malloc'_i$ we have:
		\begin{align*}
			\valu(\malloc'_i \setminus \{\good\})
			&\le \vfather{\malloc}{\malloc}{i}  & \mbox{Precondition of Rule 2}\\
			&\le \vfather{\malloc'}{\malloc'}{i}. & \mbox{Lemma \ref{p2-phase1-u2-induction}}
		\end{align*}
	\end{itemize}
	Therefore,  $\malloc'$ satisfies Property \ref{efx-father}.
\end{proof}

\begin{lemma}\label{tl:1}
		After applying Update Rule 2, we have $\phi(\malloc') > \phi(\malloc)$.
\end{lemma}
\begin{proof}
	During applying Rule 2, bundle $\malloc_{\father_{\malloc, i}}$ is returned back to the pool and bundle $\malloc'_i$ is added to the allocation. Hence we have $
		\phi(\malloc') = \phi(\malloc) - \valufather + \valu(\malloc'_i) > \phi(\malloc).
$
\end{proof}


==> src/case4/phase2-cases.tex <==
\subsubsection{Allocation Algorithm}
Our allocation algorithm in the second phase consists of $n$ steps. 
At each one of the first $n-1$ steps, we proceed as follows. We find the component with the smallest index, $l$, satisfying $1 \le l \le k$ and $|\comp_l| \ge 1$. An agent, $i$, is then selected from this component based on the following cases. We finalize The bundle of the selected agent  and move her to $\comp_0$.

\begin{itemize}
	\item \textbf{Case 1.1, There is an agent $i \in \comp_l$ such that $i$ does not have any outgoing edge in $\phasetgraph$ and $\valu_i(\malloc_i) \ge \valu_i(\malloc_0)$:}
	we finalize the bundle of agent $i$ without any further changes.
	\item \textbf{Case 1.2, There exist an agent $i \in \comp_l$ such that $i$ does not have any outgoing edge in $\phasetgraph$ and $\valu_i(\malloc_i) < \valu_i(\malloc_0)$:}
	Let $\ptpath$ be that path from agent $\repagent_l$ to agent $i$. Then for every edge $j \rightarrow j' \in \ptpath$, we set $\malloc'_j = \malloc_{j'}$. Additionally we set $\malloc'_i = \relevant_i(\malloc_0)$ and return $\malloc_i$ to the pool. Finally we move agent $i$ to the set of satisfied agents and set $\repagent'_l$ to the previous agent of agent $i$ in the path $\ptpath$.\\ %\alireza{if there is such agent, o.w $\comp'_l = \emptyset$} \alireza{$i$ has at most one incoming edge and $\repagent'_l$ is set to this incoming edge} \\
	In the following two cases each agent in $\comp_l$ has precisely one outgoing edge which is also in $\comp_l$ and vertices in $\comp_l$ form a cycle denoted by $\cycle$. For these two cases, we refer to agent $j$ as the successor of agent $i$ in the cycle, and agent $j'$ as the predecessor of agent $i$ in cycle $\cycle$.
	\item \textbf{Case 2.1, $\valu_i(\malloc_0 \cup \malloc_i) \ge \valu_i(\malloc_j)$:} In this case we set $\malloc'_i = \malloc_i \cup \relevant_i(\malloc_0)$. Then we finalize her bundle and move agent $i$ to the set of satisfied agents. Finally we set $\repagent'_l = j$.
	\item \textbf{Case 2.2, $\valu_i(\malloc_0 \cup \malloc_i) < \valu_i(\malloc_j)$:} In this case we transfer bundles through the cycle formed by agents in $\comp_l$. i.e., for every edge $t \rightarrow t' \in \cycle$ we set $\malloc'_t = \malloc_{t'}$. Then we set $\repagent'_l = j'$.
\end{itemize}
In Lemma \ref{phase2-cases-lemma} we show that after each one of the first $n-1$ steps, the allocation satisfies all the desired properties.
\begin{lemma} \label{phase2-cases-lemma}
	After each step, the resulting configuration $\conf' = (\malloc', \comp', \repagent')$ satisfies all the properties.
\end{lemma}
\begin{proof}
	Let $\conf = (\malloc, \comp, \repagent)$ be the allocation before this step and $\conf' = (\malloc', \comp', \repagent')$ be the allocation after this step.
	For each case, we prove the properties separately.
	
	\noindent
	\textbf{Case 1.1:}
	
	In this case, the bundle of all agents remains the same as before, and the only change is moving agent $i$ to the set of satisfied agents. Hence, Properties \ref{ph2-same-type}, \ref{ph2-happier}, \ref{ph2-envy-pool-type} and \ref{ph2-efx-repvalue} hold trivially.
	\begin{itemize}
		\setlength\itemsep{0.5em}
		\item \textbf{Property \ref{ph2-repagent}:} There are no outgoing edges for agent $i$, which means that there is no other agent $j$ in the same component as $i$ such that $i$ appears in the path from $\repagent_l$ to $j$. Thus, when agent $i$ is moved to $\comp_0$, there will still be a path from $\repagent'_l$ to any agent $j \in \comp'_l$ in $\phasetgraph---'$ that only contains agents of set $\comp'_l$. Furthermore since $\repagent_l$, $\malloc_{\repagent_l}$ and $\malloc_0$ are still the same as before $\conf'$ satisfies Property \ref{ph2-repagent}
		
		\item \textbf{Property \ref{ph2-component}:} Given that the allocation remains unchanged, it follows that $\ptgraph$ and $\nptgraph$ are identical. Therefore the property clearly holds.
		
		\item \textbf{Property \ref{ph2-satisfied}:} Since agent $i$ does not have any outgoing edge in $\phasetgraph$, there is not any other agent $j \notin \comp_0$, $j \ne i$ such that $\valu_i(\malloc_0) > 0$. Therefore we have:
		\begin{align*}
			\valu_i( \bigcup\limits_{j \notin \comp'_0 \lor j = 0} \malloc'_j) &= \valu_i(\malloc_0) \\
			&\le \valu_i(\malloc_i) & \mbox{Conditions of Case 1.1} \\
			&= \valu_i(\malloc'_i) & \mbox{Bundles do not change}
		\end{align*}
		
		\item \textbf{Property \ref{ph2-efx-satisfied}:} After this step agent $i$ will be added to $\comp'_0$. As $\conf$ satisfies Property \ref{ph2-satisfied}, no agent $j \in \comp_0$ envies agent $i$. Therefore it is sufficient to show that $i$ does not strongly envy any agent $j \in \comp_0$ after this step. Hence, for every agent $j \in \comp_0$ and good $\good \in \malloc'_j$ we have the following:
		\begin{align*}
			\valu_i(\malloc'_j \setminus \{\good\}) &= \valu_i(\malloc_j \setminus \{\good\}) &\mbox{$\malloc'_j = \malloc_j$}\\
			&\le \repvalu_i & \mbox{$\conf$ satisfies \ref{ph2-efx-repvalue}} \\
			&\le \valu_i(\malloc_i) & \mbox{$\conf$ satisfies \ref{ph2-happier}} \\
			&= \valu_i(\malloc'_i) & \mbox{$\malloc'_i = \malloc_i$} \\
		\end{align*}
	\end{itemize}
	
	\noindent
	\textbf{Case 1.2:}
	
	In this case, the bundles of agents in $\ptpath$ are transferred through the path. After that $\malloc'_i$ is set to $\relevant_i(\malloc_{0})$ and agent $i$ moved to the set of satisfied agents. Furthermore $\malloc_{\repagent_l}$ is returned to the pool. Note that the bundle of agents not in the path remains the same as before.
	\begin{itemize}
		\setlength\itemsep{0.5em}
		\item \textbf{Property \ref{ph2-same-type}:} For any agent $j \notin \comp'_0$ that is not included in path $\ptpath$, $\malloc'_j = \malloc_j$ and since $\conf$ satisfies Property \ref{ph2-same-type} the property holds trivially. In addition, for those agents who belong to path $\ptpath$ but not to $\comp'_0$  since agent $i$ is moved to $\comp'_0$ during this step, we have $j \ne i$, therefore there exist an agent $j'$ such that $j \rightarrow j' \in \ptpath$ and $\malloc'_j = \malloc_{j'}$. Furthermore since all the goods in $\malloc_{j'}$ are relevant to both agents $j$ and $j'$ we have $\malloc'_j = \malloc_{j'} \subseteq \edge_{j, j'}$ and $\conf'$ satisfies Property \ref{ph2-same-type}.
		
		\item  \textbf{Property \ref{ph2-repagent}:} This step results in the reversal of the edges in path $\ptpath$. The reason is straightforward: for every edge $j \rightarrow j' \in \ptpath$, we have $\malloc'_j = \malloc_{j'}$, and the goods in $\malloc'_j$ are relevant to agent $j'$. Consequently, an edge is formed from agent $j'$ to agent $j$ in $\nptgraph$. In addition, $\repagent'_l$ is set to the predecessor agent of agent $i$ in path $\ptpath$. Since agent $i$ has no outgoing edges in $\phasetgraph$ and has been removed from $\comp'_l$ in this step, along with the reversal of the direction of the edges, we can infer that agent $\repagent'_l$ has a path to any other agent in $\comp'_l$ that only includes agents belonging to $\comp'_l$. 
		
		Furthermore, it should be noted that $\malloc'_{\repagent'_l} = \malloc_i$ and the goods in this bundle are relevant to both agents $\repagent'_l$ and $i$. Also, $\malloc'_i = \relevant_i(\malloc_0)$ and the bundle $\malloc_{\repagent_l}$ which is returned to the pool in this step does not have any good that is relevant to agent $i$ since agent $i$ has no outgoing edge in $\phasetgraph$. Therefore, all the goods in $\malloc'_0$ are irrelevant to agent $i$, and $\malloc'_0 \cap \edge_{\repagent'_l, i} = \emptyset$. Hence, there is no good $\good \in \malloc'_0$ for which $\malloc'_{\repagent'_l} \cup \{\good\} \subseteq \edge_{\repagent'_l, i}$. Additionally, agent $\repagent'_l$ has no incoming edges in $\phasetgraph----{\conf'}$ since its only incoming edge in $\nptgraph$ is from agent $i$, which is transferred to $\comp'_0$ in this step. Thus $\conf'$ satisfies Property \ref{ph2-repagent}.
		
		\item  \textbf{Property \ref{ph2-component}:} For all components $\comp_{l'}$ such that $l < l' \le k$, the agents and their bundles remain unchanged. Therefore, since $\conf$ satisfies \ref{ph2-component}, this property still holds after this step.
		
		\item  \textbf{Property \ref{ph2-happier}:} It is sufficient to show that the property holds for every agent $j \notin \comp'_0$ whose bundle changes in this step. This means that $j$ must be a part of path $\ptpath$, but not the same agent as $i$. Additionally, there must be another agent $j'$ such that $j \rightarrow j' \in \ptpath$ and $\malloc'_j = \malloc_{j'}$. As both agents are in the component $\comp_l$, according to Observation \ref{same-repvalue} we can conclude that $\repvalu_j = \repvalu_{j'}$. Therefore we have the following:
		\begin{align*}
			\valu_j(\malloc'_j) &= \valu_{j'}(\malloc_{j'}) &\mbox{Goods in $\malloc'_j$ are relevant to both $j$ and $j'$}\\
			&\ge \repvalu_{j'} & \mbox{$\conf$ satisfies \ref{ph2-happier}} \\
			&= \repvalu_j & \mbox{Observation \ref{same-repvalue}} \\
		\end{align*}
		
		\item  \textbf{Property \ref{ph2-envy-pool-type}:} The only goods that are returned to the pool are those that are in bundle $\malloc_{\repagent_l}$. If $\malloc_{\repagent_l} = \emptyset$, then this property holds trivially since $\conf$ satisfies Property \ref{ph2-envy-pool-type}. Let $j$ be the agent such that $\malloc_{\repagent_l} \subseteq \edge_{\repagent_l, j}$. It is sufficient to show that this property holds for agents $\repagent_l$ and $j$. We do not need to check this property if at least one of them is in $\comp'_0$. Therefore, we have $j, \repagent_l \notin \comp'_0$. We know that $l$ is the minimum index where $\comp_l$ is not empty. This implies that $\repvalu_{\repagent_l} \le \repvalu_j$, and there exists an edge from agent $j$ to agent $\repagent_l$ in $\phasetgraph$ because the goods in $\malloc_{\repagent_l}$ are relevant to agent $j$. Furthermore, since $\conf$ satisfies Property \ref{ph2-repagent}, we can conclude that $\malloc_0 \cap \edge_{\repagent_l, j} = \emptyset$. Additionally, since $\repagent_l$ has an incoming edge in $\phasetgraph$, we have $\valu(\malloc_{\repagent_l}) = \repvalu_l$. Hence we have the following:
		\begin{align*}
			\valu(\malloc'_0 \cap \edge_{\repagent_l, j}) &\le \valu((\malloc_0 \cup \malloc_{\repagent_l}) \cap \edge_{\repagent_l, j}) \\% &\mbox{Only the goods in $\malloc_{\repagent_l}$ are returned to the pool}\\
			&= \valu((\malloc_0 \cap \edge_{\repagent_l, j}) \cup (\malloc_{\repagent_l} \cap \edge_{\repagent_l, j})) \\
			&= \valu(\malloc_{\repagent_l}) &\mbox{$\malloc_0 \cap \edge_{\repagent_l, j} = \emptyset$ and $\malloc_{\repagent_l} \subseteq \edge_{\repagent_l, j}$} \\
			&= \repvalu_{\repagent_l} &\mbox{$\repagent_l$ has an incoming edge in $\phasetgraph$}
		\end{align*}
		Therefore $\valu(\malloc'_0 \cap \edge_{\repagent_l, j}) \le \repvalu_{\repagent_l} \le \repvalu_j$ and $\conf'$ satisfies Property \ref{ph2-envy-pool-type}.
		
		\item \textbf{Property \ref{ph2-efx-repvalue}:} As we transfer the bundles along $\ptpath$, every bundle in $\malloc'$, except the bundle of agent $i$, matches a bundle in $\malloc$ that may belong to another agent. Thus, it is enough to prove that for every agent $j \notin \comp'_0$ and good $\good \in \malloc'_i$ we have $\valu_j(\malloc'_i \setminus \{\good\}) \le \repvalu_j$.
		\begin{align*}
			\valu_j(\malloc'_i \setminus \{\good\}) &\le \valu_j(\malloc'_i) \\% &\mbox{Only the goods in $\malloc_{\repagent_l}$ are returned to the pool}\\
			&= \valu_j(\relevant_i(\malloc_0)) &\mbox{$\malloc'_i = \relevant_i(\malloc_0)$} \\
			&= \valu(\malloc_0 \cap \edge_{i, j}) &\mbox{Relevant to both $i$ and $j$} \\
			&\le \repvalu_j &\mbox{$\conf$ satisfies Property \ref{ph2-envy-pool-type}}
		\end{align*}
		Hence $\valu_j(\malloc'_i \setminus \{\good\}) \le \repvalu_j$ and Property \ref{ph2-efx-repvalue} holds.
		
		\item \textbf{Property \ref{ph2-satisfied}:}  To demonstrate that the configuration $\conf'$ satisfies Property \ref{ph2-satisfied}, we can focus solely on agent $i$. This is because agent $i$ is the only agent that has been moved to the set of satisfied agents. Since agent $i$ does not have any outgoing edge, the only remaining bundles with at least one relevant good to agent $i$ are $\malloc_0$ and $\malloc_i$. Furthermore since $\malloc'_i = \relevant_i(\malloc_0)$ all the goods in $\malloc_0$ that are relevant to agent $i$ are allocated to this agent we have the following:
		\begin{align*}
			\valu_i( \bigcup\limits_{j \notin \comp'_0 \lor j = 0} \malloc'_j) &= \valu_i(\malloc_i) \\
			&< \valu_i(\malloc_0) & \mbox{Conditions of Case 1.2} \\
			&= \valu_i(\relevant_i(\malloc_0)) \\
			&= \valu_i(\malloc'_i) &\mbox{$\malloc'_i = \relevant_i(\malloc_{0})$}
		\end{align*}
		Thus $\conf'$ satisfies Property \ref{ph2-satisfied}.
		
		\item \textbf{Property \ref{ph2-efx-satisfied}:} Agent $i$ is the only agent moved to $\comp'_0$. As $\conf$ satisfies Property \ref{ph2-satisfied}, no agent $j \in \comp_0$ envies agent $i$. Therefore, it is sufficient to show that agent $i$ does not strongly envy any agent $j \in \comp_0$. For every agent $j \in \comp_0$ and good $\good \in \malloc'_j$ we have:
		\begin{align*}
			\valu_i(\malloc'_j \setminus \{\good\}) &= \valu_i(\malloc_j \setminus \{\good\}) &\mbox{$\malloc'_j = \malloc_j$}\\
			& \le \repvalu_i & \mbox{$\conf$ satisfies Property \ref{ph2-efx-repvalue}} \\
			&\le \valu_i(\malloc_i) & \mbox{$\conf$ satisfies Property \ref{ph2-happier}} \\
			&\le \valu_i(\malloc_0) &\mbox{Condition of Case 1.2} \\
			&= \valu_i(\relevant_i(\malloc_0)) \\
			&= \valu_i(\malloc'_i) &\mbox{$\malloc'_i = \relevant_i(\malloc_0)$}
		\end{align*}
	\end{itemize}
	
	\noindent
	\textbf{Case 2.1:}
	
	In this case, the bundle of all agents except agent $i$ remains the same as before. Furthermore, agent $i$ is now moved to the set of satisfied agents. Note that since $\malloc'_i = \malloc_i \cup \relevant_i(\malloc_0)$ we have $\malloc'_0 \subseteq \malloc_0$. Therefore, Properties \ref{ph2-same-type}, \ref{ph2-happier}, and \ref{ph2-envy-pool-type} hold trivially.
	\begin{itemize}
		\setlength\itemsep{0.5em}
		\item \textbf{Property \ref{ph2-repagent}:} Since agents in $\comp_l$ form a cycle, after removing agent $i$ from component $\comp_l$ and adding it to $\comp'_0$, the resulting graph still has a path from agent $\repagent'_l=j$ to any other agent in $\comp'_l$. 
		
		Additionally, since goods in $\malloc'_j$ are relevant to both agents $i$ and $j$, agent $i$ is the only incoming edge of agent $j$ in $\nptgraph$ who is moved to $\comp'_0$. Hence, agent $j$ has no incoming edge in $\phasetgraph----{\conf'}$. Moreover since $\malloc'_i = \malloc_i \cup \relevant_i(\malloc_0)$, $\malloc'_0$ does not contain a good that is relevant to agent $i$ and there is no good $\good \in \malloc'_0$ such that $\malloc'_j \cup \{\good\} \subseteq \edge_{i, j}$. Therefore $\conf'$ satisfies Property \ref{ph2-repagent}.
		
		\item \textbf{Property \ref{ph2-component}:} Bundles of agents not in $\comp'_0$ remain unchanged. Thus, this property holds trivially.
		
		\item \textbf{Property \ref{ph2-efx-repvalue}:} 
		The only changed bundle is the bundle of agent $i$. Hence, we only need to prove the condition for every agent $t \notin \comp'_0$ and good $\good \in \malloc'_i$. Since agent $i$ is the representative agent of component $\comp_l$ and $\conf$ satisfies Property \ref{ph2-repagent}, we have $\valu(\malloc_i) = \repvalu_i$.  
		
		Additionally, since goods in $\malloc_i$ are relevant to both agents $i$ and $j'$ and $\conf$ satisfies Property \ref{ph2-repagent}, there can be no good $\good$ in $\malloc_0$ that is relevant to both agents $i$ and $j'$. Therefore for agent $j'$ we have:
		\begin{align*}
			\valu_{j'}(\malloc'_i \setminus \{\good\}) &\le \valu_{j'}(\malloc'_i) \\% &\mbox{Only the goods in $\malloc_{\repagent_l}$ are returned to the pool}\\
			&= \valu_{j'}(\malloc_i \cup \relevant_i(\malloc_0)) &\mbox{$\malloc'_i = \malloc_i \cup \relevant_i(\malloc_0)$} \\
			&= \valu_{j'}(\malloc_i) &\mbox{$\malloc_0 \cap \edge_{i, j'} = \emptyset$} \\
			&= \valu(\malloc_i) &\mbox{Relevant to agent $j'$} \\
			&= \repvalu_i &\mbox{$\conf$ satisfies Property \ref{ph2-repagent}} \\
			&= \repvalu_{j'} &\mbox{$j' \in \comp_l$ and Observation \ref{same-repvalue}}
		\end{align*}
		Furthermore, for the agents $t \notin \comp'_0$ and $t \ne j'$, goods in $\malloc_i$ are not relevant to agent $t$. Therefore we have:
		\begin{align*}
			\valu_t(\malloc'_i \setminus \{\good\}) &\le \valu_t(\malloc'_i) \\% &\mbox{Only the goods in $\malloc_{\repagent_l}$ are returned to the pool}\\
			&= \valu_t(\malloc_i \cup \relevant_i(\malloc_0)) &\mbox{$\malloc'_i = \malloc_i \cup \relevant_i(\malloc_0)$} \\
			&= \valu_t(\relevant_i(\malloc_0)) &\mbox{$\valu_t(\malloc_i) = 0$} \\
			&= \valu(\malloc_0 \cap \edge_{i, t}) &\mbox{Relevant goods to both agent $i$ and $t$} \\
			&\le \repvalu_t &\mbox{$\conf$ satisfies Property \ref{ph2-envy-pool-type}}. \\
		\end{align*}
		Hence $\conf'$ satisfies Property \ref{ph2-efx-repvalue}.
		
		\item \textbf{Property \ref{ph2-satisfied}:} In this step, only agent $i$ has been moved to $\comp'_0$. Hence, it is sufficient to prove this property for agent $i$. As the only outgoing edge of agent $i$ is towards agent $j$, bundles $\malloc_i$, $\malloc_j$, and $\malloc_0$ are the only ones that have at least one good relevant to agent $i$. Moreover, since $\malloc'_i = \malloc_i \cup \relevant_i(\malloc_0)$, all the goods in $\malloc_i$ and $\malloc_0$ that are relevant to agent $i$ are allocated to her. Therefore, the only remaining bundle with at least one good that is relevant to agent $i$ is $\malloc_j$, and thus we can conclude that:
		\begin{align*}
			\valu_i( \bigcup\limits_{j \notin \comp'_0 \lor j = 0} \malloc'_j) &= \valu_i(\malloc_j) \\
			&\le \valu_i(\malloc_i \cup \malloc_0) & \mbox{Conditions of Case 2.1} \\
			&= \valu_i(\malloc_i \cup \relevant_i(\malloc_0)) \\
			&= \valu_i(\malloc'_i) &\mbox{$\malloc'_i = \malloc_i \cup \relevant_i(\malloc_0)$}
		\end{align*}
		
		\item \textbf{Property \ref{ph2-efx-satisfied}:} Since $\conf$ satisfies Property \ref{ph2-satisfied}, there is no agent $t \in \comp_0$ who envies agent $i$. Furthermore for every agent $t \in \comp_0$ and $\good \in \malloc'_t$ we have:
		\begin{align*}
			\valu_i(\malloc'_t \setminus \{\good\}) &= \valu_i(\malloc_t \setminus \{\good\}) &\mbox{$\malloc'_t = \malloc_t$}\\
			& \le \repvalu_i & \mbox{$\conf$ satisfies Property \ref{ph2-efx-repvalue}} \\
			&\le \valu_i(\malloc_i) & \mbox{$\conf$ satisfies Property \ref{ph2-happier}} \\
			&\le \valu_i(\malloc_i \cup \relevant_i(\malloc_0)) \\
			&= \valu_i(\malloc'_i) &\mbox{$\malloc'_i = \malloc_i \cup \relevant_i(\malloc_0)$}
		\end{align*}
		Therefore there is no agent $t \in \comp_0$ such that $i$ strongly envies agent $t$ and Property \ref{ph2-efx-satisfied} holds.
	\end{itemize}
	
	\noindent
	\textbf{Case 2.2:}
	
	In this case, the bundles of agents in $\cycle$ are transferred through the cycle. Then we finalize bundle of agent $i$ and move it to $\comp'_0$. Finally we set $\repagent'_l = j'$. It should be noted that as we transferred the bundle through the cycle, each bundle in $\malloc$ is identical to a bundle in $\malloc'$ that may be owned by a different agent. Therefore the Properties \ref{ph2-envy-pool-type} and \ref{ph2-efx-repvalue} hold trivially.
	\begin{itemize}
		\item \textbf{Property \ref{ph2-same-type}:} The property holds for agents whose bundle remains unchanged since $\conf$ satisfies Property \ref{ph2-same-type}. Let $t$ be an agent in the cycle. There exist another agent $t'$ such that $t \rightarrow t' \in \cycle$ and then $\malloc'_t = \malloc_{t'}$. Therefore, since the goods in bundle $\malloc'_t$ are relevant to both agents $t$ and $t'$, it implies that $\malloc'_t \subseteq \edge_{t, t'}$ and Property \ref{ph2-same-type} holds.
		
		\item \textbf{Property \ref{ph2-repagent}:} After transferring bundles through cycle $\cycle$, the edges in $\cycle$ will have their directions reversed. Suppose $t \rightarrow t' \in \cycle$ is an edge in the cycle. After this step, $\malloc'_t = \malloc_{t'}$ and the goods in $\malloc'_t$ are now relevant to agent $t'$. As a result, an edge now exists from agent $t'$ to agent $t$ in $\nptgraph$. Therefore, we can conclude that after removing agent $i$ from $\comp_l$, there will be a path from $\repagent'_l = j'$ to any other agent in $\comp'_l$ that consists only agents in $\comp'_l$.
		
		Additionally, since $\malloc'_{j'} = \malloc_i$ and $\malloc'_0 = \malloc_0$, and $\conf$ satisfies Property \ref{ph2-repagent}, there does not exist a good $\good \in \malloc'_0$ such that $\malloc'_{j'} \cup \{\good\} \subseteq \edge_{i, j'}$.
		Moreover the only incoming edge of agent $j'$ in $\nptgraph$ is from agent $i$ which is moved to $\comp'_0$ in this step. Therefore $j'$ does not have any incoming edge in $\phasetgraph-----{\conf'}$ and $\conf'$ satisfies Property \ref{ph2-repagent}.
		
		\item \textbf{Property \ref{ph2-component}:} %\alireza{TODO: Rephrase, copy pasted from case 1.2}
		For all components $\comp_{l'}$ such that $l < l' \le k$, the agents and their bundles remain unchanged. Therefore, since $\conf$ satisfies \ref{ph2-component}, this property still holds after this step.
		
		\item \textbf{Property \ref{ph2-happier}:} For those agents whose bundle remains unchanged, this property holds trivially. Let $t$ be an agent in the cycle. There is another agent $t'$ such that $t \rightarrow t' \in \cycle$ and $\malloc'_t = \malloc_{t'}$. We can conclude from Observation \ref{same-repvalue} that $\repvalu_{t} = \repvalu_{t'}$. Therefore we have:
		\begin{align*}
			\valu_t(\malloc'_t) &= \valu_{t'}(\malloc_{t'}) &\mbox{Goods in $\malloc'_t$ are relevant to both $t$ and $t'$}\\
			&\ge \repvalu_{t'} & \mbox{$\conf$ satisfies \ref{ph2-happier}} \\
			&= \repvalu_t & \mbox{Observation \ref{same-repvalue}} \\
		\end{align*}
		
		\item \textbf{Property \ref{ph2-satisfied}:} Since agent $i$ is the only agent moved to $\comp'_0$, we only need to prove this statement for agent $i$. It is important to note that there are only three bundles that contain goods relevant to agent $i$: $\malloc_i$, $\malloc_j$, and $\malloc_0$. Given that $\malloc'_i = \malloc_j$, it leaves us with only two bundles that have at least one relevant good for agent $i$: $\malloc_i$ and $\malloc_0$. Therefore we have:
		\begin{align*}
			\valu_i( \bigcup\limits_{j \notin \comp'_0 \lor j = 0} \malloc'_j) &= \valu_i(\malloc_i \cup \malloc_0) \\
			&< \valu_i(\malloc_j) & \mbox{Conditions of Case 2.2} \\
			&= \valu_i(\malloc'_i) &\mbox{$\malloc'_i = \malloc_j$}
		\end{align*}
		Thus $\conf'$ satisfies Property \ref{ph2-satisfied}.
		
		\item \textbf{Property \ref{ph2-efx-satisfied}:} It is sufficient to show that $i$ does not strongly envy any agent $t \in \comp_0$ and there is no agent $t \in \comp_0$ who strongly 	envies agent $i$. Since $\conf$ satisfies Property \ref{ph2-efx-satisfied}, there does not exist an agent $t \in \comp_0$ such that $t$ envies agent $i$. Furthermore for every agent $t \in \comp_0$ and good $\good \in \malloc'_t$ we have:
		\begin{align*}
			\valu_i(\malloc'_t \setminus \{\good\}) &= \valu_i(\malloc_t \setminus \{\good\}) &\mbox{$\malloc'_t = \malloc_t$ since $t \in \comp_0$}\\
			& \le \repvalu_i & \mbox{$\conf$ satisfies Property \ref{ph2-efx-repvalue}} \\
			&\le \valu_i(\malloc_i) & \mbox{$\conf$ satisfies Property \ref{ph2-happier}} \\
			&\le \valu_i(\malloc_i \cup \malloc_0) \\
			&\le \valu_i(\malloc_j) &\mbox{Condition of Case 2.2} \\
			&= \valu_i(\malloc'_i) &\mbox{$\malloc'_i = \malloc_j$}
		\end{align*}
	\end{itemize}
	
	Thus the resulting configuration $\conf'$ satisfies all the properties.
\end{proof}

\textbf{Final Step:} After $n-1$ steps, we allocate all the remaining goods, to the only remaining agent who has not yet been satisfied and terminate the algorithm. Algorithm \ref{alg:phase2} provides a pseudocode of our allocation algorithm in the second phase.

\begin{theorem} \label{phase2-efx-lemma}
	Let $\malloc$ be the allocation after $n$'th step. Then, $\malloc$ is $\efx$.
\end{theorem}
\begin{proof}
	Let $i$ be the only remaining agent such that $i \notin \comp_0$. In the final step we allocate all the remaining goods to agent $i$. i.e., we set $\malloc'_i = \malloc_i \cup \malloc_0$. Since $\conf$ satisfies Property \ref{ph2-satisfied}, there is no agent $j \in \comp_0$ such that $j$ envies agent $i$. Furthermore for every agent $j \in \comp_0$ and good $\good \in \malloc'_j$ we have:
	\begin{align*}
		\valu_i(\malloc'_j \setminus \{\good\}) &= \valu_i(\malloc_j \setminus \{\good\}) &\mbox{$\malloc'_j = \malloc_j$ since $j \in \comp_0$}\\
		& \le \repvalu_i & \mbox{$\conf$ satisfies Property \ref{ph2-efx-repvalue}} \\
		&\le \valu_i(\malloc_i) & \mbox{$\conf$ satisfies Property \ref{ph2-happier}} \\
		&\le \valu_i(\malloc_i \cup \malloc_0) \\
		&= \valu_i(\malloc'_i) &\mbox{$\malloc'_i = \malloc_i \cup \malloc_0$}
	\end{align*}
	Thus, agent $i$ does not strongly envy any agent $j \in \comp_0$. Additionally, since $\conf$ satisfies Property \ref{ph2-efx-satisfied}, there are no two agents $j, j' \in \comp_0$ such that $j$ strongly envies $j'$. Therefore, there is no strong-envy in $\malloc'$, and allocation $\malloc'$ is $\efx$.
\end{proof}

==> src/case4/phase2-code.tex <==
\begin{algorithm}
	\KwIn{An allocation $\malloc$ satisfies properties \ref{same-type} and \ref{efx-father} such that Update Rules 1 and 2 of Phase 1 are not applicable}
	\KwOut{A complete $\efx$ allocation}
	Let $\repagent = \repagent_1, \repagent_2, \dots \repagent_k$ be the agents such that $\father_{\malloc, \repagent_i} = \repagent_i$ and 
	$(\valu(\malloc_{\repagent_1)}, \repagent_1) < (\valu(\malloc_{\repagent_2)}, \repagent_2), \dots (\valu(\malloc_{\repagent_k)}, \repagent_k)$ \\
	\For{$i\gets1$ \KwTo $k$}{
	$\repvalu_i \leftarrow \valu(\malloc_{\repagent_i})$. \tcp*{$\repvalu_i$ is constant during the algorithm.}
	}
	\For{$i\gets1$ \KwTo $k$}{
		$\comp_i \gets \{j \mid \father_{\malloc, j} = \repagent_i$\texttt{}\}
	}
	 $\comp_0 \gets \emptyset$.\\
	 $\conf \gets (\malloc, \comp, \repagent)$\\
	\Repeat{$n- 1$ times}{
		Let $\phasetgraph \gets$ $\ptgraph\setminus\comp_0$.\\
		 $l\gets$  $\min_{1 \le i \le k,|\comp_i| >0 } i$.\\
		\If{$\exists i \in \comp_l$ such that $i$ does not have outgoing edge in $\phasetgraph$}{
			\If{$\valu(\malloc_i) \ge \valu_i(\malloc_{0})$}{
				 $\comp'_l \gets \comp_l \setminus \{i\}$. \\
				$\comp'_0 \gets \comp_0 \cup \{i\}$.
			}
			\Else{
				Transfer bundles through the path from $\repagent_l$ to $i$ in $\phasetgraph$. \\
				 $\malloc'_i \gets \relevant_i(\malloc_i)$. \\
				 $\malloc'_0 \gets (\malloc_0 \setminus \relevant_i(\malloc_i)) \cup \malloc_{\repagent_l}$. \\
				If $|\comp_l| \ge 2$, set $\repagent'_l$ to the previous agent in the from $\repagent_l$ to $i$\\ 
				 $\comp'_l \gets \comp_l \setminus \{i\}$. \\
				 $\comp'_0 \gets \comp_0 \cup \{i\}$.
			}
		}
		\Else{
			In this case vertices in $\comp_l$ form a cycle in $\phasetgraph$ denoted by $\cycle$.\\
			Let $i$ be $\repagent_l$, $j$ be the successor agent of agent $i$ in $\cycle$ and $j'$ be the predecessor agent of agent $i$ in $\cycle$ \\
			\If{$\valu_i(\malloc_0 \cup \malloc_i) \ge \valu_i(\malloc_j)$ }{
				 $\malloc'_i \gets \malloc_i \cup \relevant_i(\malloc_i)$.\\
				 $\malloc'_0 \gets \malloc_0 \setminus \relevant_i(\malloc_i)$. \\
				 $\repagent'_l \gets j$. \\
				 $\comp'_l \gets \comp_l \setminus \{i\}$. \\
				 $\comp'_0 \gets \comp_0 \cup \{i\}$.
			}
			\Else{
				$\repagent'_l \gets j'$\\
				Transfer the bundles through cycle $\cycle$. \\
				 $\comp'_l \gets \comp_l \setminus \{i\}$. \\
				 $\comp'_0 \gets \comp_0 \cup \{i\}$.
			}
		}
		 $\conf \gets (\malloc', \comp', \repagent')$.\\
	}
	Let $i = \agents \setminus \comp_0$. \\
	 $\malloc'_i \gets \malloc_i \cup \malloc_0$. \\
	\Return{$\malloc'$}
	\caption{Phase 2 Allocation Algorithm}
	\label{alg:phase2}
\end{algorithm}
\newpage

==> src/case4/phase2-intro.tex <==
\subsection{Phase 2}
When none of the rules in the first phase is applicable, we proceed to the second phase. The objective of this phase is to allocate all the remaining goods so that the resulting allocation is $\efx$.
This phase comprises $n - 1$ steps, followed by a final step. In each of these $n - 1$ steps, we take a triple $\conf = (\malloc, \comp, \repagent)$ as input and return another triple $\conf' = (\malloc', \comp', \repagent')$. Here, $\malloc = \langle \malloc_0, \malloc_1, \dots, \malloc_n \rangle$ represents the allocation, and $\comp = \langle \comp_0, \comp_1, \dots, \comp_k \rangle$ represents a partitioning of agents. Specifically, each $\comp_i$ is a subset of agents. The agents in $\comp_0$ are satisfied agents. Additionally, we designate one agent in $\comp_i$ as the representative of $\comp_i$ and denote them by $\repagent_i$.
Finally, for each agent $i$, we assign a value $\repvalu_i$, referred to as the representative value of agent $i$. This value remains constant throughout the entire second phase.

The second phase's initial configuration builds upon the allocation $\malloc$ obtained from the first phase as follows:
\begin{itemize}
	\item We let $r = [r_1,r_2,\ldots,r_k]$ to be the vector of root agents, sorted by their bundle values, i.e., $\valu(\malloc_{\repagent_1}) \leq \valu(\malloc_{\repagent_2}) \leq \ldots \leq \valu(\malloc_{\repagent_k})$. In the event of equal values, the agent with the smaller index comes first.
	\item For each agent $i$, we set $\repvalu_i = \valufather$.  
	\item 
	For each $1 \le l \le k$, $\comp_l$ is  the set of agents $i$ for which $\father_{\malloc, i} = \repagent_l$. $\comp_0$ is empty.
		
\end{itemize}

During each of the $n - 1$ steps, we find the smallest index $l$ such that $\comp_l $ is not empty. Next, we select one agent from $\comp_l$, finalize her bundle and move it to the set of satisfied agents. For brevity we denote by $\phasetgraph$, an induced subgraph of $\ptgraph$, comprising only those agents who have not yet been satisfied. 
We perform these updates in a way that the configuration satisfies all the following conditions during the second phase:



\begin{enumerate} [label=\textcolor{red}{$\zeta\!\!$} (\roman*)]
	\item \label{ph2-same-type} For every agent $i \notin \comp_0$, there exist an agent $j$ such that $\malloc_i \subseteq \relevant {\goods}{i,j}$. 
	\item \label{ph2-repagent} For every non-empty component $\comp_l$ and agent $i \in \comp_l$, there exist a path from $\repagent_l$ to agent $i$ in $\phasetgraph$ that only contains agents of $\comp_l$. Moreover there is no agent $j$ and good $\good \in \malloc_0$ such that $\malloc_{\repagent_l} \cup {\good} \subseteq \relevant{\goods}{\repagent_l, j}$. Additionally if $\repagent_l$ has incoming edge in $\phasetgraph$ we have $\valu(\malloc_{\repagent_l}) = \repvalu_{\repagent_l}$. 
	\item \label{ph2-component} For every two agent $i \in \comp_l$ and $ j \in \comp_{l'}$ such that $1 \le l < l' $, we have $\valu_i(\malloc_j) = 0$. 
	\item \label{ph2-happier} For every agent $i \notin \comp_0$, $\valu(\malloc_i) \ge \repvalu_i$.
	\item \label{ph2-envy-pool-type} For every two agents $i, j \notin \comp_0$ and $i \ne j$ we have: $\valu(\malloc_0 \cap \relevant{\goods}{i, j}) \le \repvalu_i$. 
	\item \label{ph2-efx-repvalue} For every agent $i \notin \comp_0$ and agent $j$ and every good $\good \in \malloc_j$ we have: $\valu_i(\malloc_j \setminus \{\good\}) \le \repvalu_i$.
	\item \label{ph2-satisfied} For every agent $i \in \comp_0$ we have: $\valu_i( \bigcup\limits_{j \notin \comp_0 \lor j = 0} \malloc_j) \le \valu_i(\malloc_i)$.  
	\item \label{ph2-efx-satisfied} For every two agents $i, j \in \comp_0$, agent $i$ does not strongly envy agent $j$.
\end{enumerate}

\begin{lemma} \label{p2-phase1-phase2-properties}
	The initial configuration $\conf = (\malloc, \comp, \repagent)$ satisfies all the properties.
\end{lemma}
\begin{proof}
	We prove each one of the properties separately.
	\begin{itemize}
		\setlength\itemsep{0.5em}
		\item \textbf{Property \ref{ph2-same-type}:} The allocation returned by the first phase, $\malloc$, satisfies Property \ref{same-type}. Therefore $\conf$ satisfies Property \ref{ph2-same-type}.
		
		\item \textbf{Property \ref{ph2-repagent}:} For every component $C_l$ and every agent $i \in \comp_l$, we have $\father_{\malloc, i} = \repagent_l$. Hence, a path exists from $\repagent_l$ to agent $i$ in $\phasetgraph$ and by Observation \ref{path-father} every agent that appears in this path is also in $\comp_l$. Furthermore since $\father_{\malloc, \repagent_l} = \repagent_l$ and the Update Rule 1 of the first phase is not applicable there does not exist an agent $j$ and good $\good \in \malloc_0$ such that $\malloc_{\repagent_l} \cup {\good} \subseteq \edge_{\repagent_l, j}$. Additionally $\repvalu_{\repagent_l} = \valu(\malloc_{\father_{\malloc, \repagent_l}}) = \valu(\malloc_{\repagent_l})$ and Property \ref{ph2-repagent} holds.
		
		\item \textbf{Property \ref{ph2-component}:} If there are two agents, $i$ and $j$  in different components, $\comp_l$ and $\comp_{l'}$ respectively, where $1 \leq l < l' \leq k$, and $\valu_i(\malloc_j) > 0$, then there must be an edge from agent $i$ to agent $j$ in the $\ptgraph$. As a result, there exists a path from agent $\repagent_l$ to agent $j$. Moreover, since $(\repagent_l, l) < (\repagent_{l'}, l')$, we can conclude that $\father_{\malloc, j} \neq \repagent_{l'}$, which contradicts the fact that $\father_{\malloc, j} = \repagent_{l'}$.
		
		\item \textbf{Property \ref{ph2-happier}:} By Observation \ref{obs-more-than-father} for each agent $i$ we have: $\valu(\malloc_i) \ge \valufather = \repvalu_i$.
		
		\item \textbf{Property \ref{ph2-envy-pool-type}:} As $\malloc$ is the allocation returned by the first phase, Update Rule 2 of this phase is not applicable. Therefore for every two agents $i \ne j$ we have $\valu(\malloc_{0} \cap \edge_{i, j}) \le \valu(\father_{\malloc, i}) = \repvalu_i$.
		
		
		\item \textbf{Property \ref{ph2-efx-repvalue}:} If $\vals_i(\malloc_j) = 0$, the property trivially holds. Otherwise all the goods in $\malloc_j$ are relevant to agent $i$ and there exist an edge from agent $i$ to agent $j$ in $\ptgraph$. Hence we have: 
		\begin{align*}
			\valu_i(\malloc_j \setminus \{\good\}) &= \valu(\malloc_j \setminus \{\good\}) & \mbox{Goods in $\malloc_j$ are relevant to agent $i$} \\
			&\le \vfather{\malloc}{\malloc}{j}  & \mbox{$\malloc$ satisfies Property \ref{efx-father}}\\
			&\le \vfather{\malloc}{\malloc}{i} & \mbox{Lemma \ref{less-father}}\\
			&= \repvalu_i & \mbox{$\repvalu_i = \valufather$}
		\end{align*}
		
		\item \textbf{Properties \ref{ph2-satisfied} and \ref{ph2-efx-satisfied}:} These properties hold trivially since $\comp_0 = \emptyset$.
	\end{itemize}
\end{proof}

==> src/case6new.tex <==
\section{$\frac{\sqrt{2}}{2}$-$\efx$ for Restricted Additive Valuations New}\label{sec:5new}
In this section, we present a $\frac{\sqrt{2}}{2}$-$\efx$ allocation algorithm for the case that the set of valuations is restricted additive. The algorithm consists of two updating rules and a final step. After each update, we use an envy elimination process to ensure the allocation remains $\invsq$-$\efx$.  Each one of the updating rules, the envy elimination process, and the final step takes an allocation as input and returns another allocation as output. 
Our algorithm ensures that, in all steps before the final step, Property \ref{prop:2new} holds. This property trivially holds for the basic feasible allocation.

\begin{enumerate}[label=\textcolor{red}{$\S\!\!$} (\roman*)]
	\item\!\!: \label{prop:2new}	For every agent $i$, $\relevant{\malloc_i}{i} = \malloc_i$. 	
\end{enumerate}


Given Lemma \ref{lem:11}, Property \ref{prop:2new} implies that $G_{\sqrt{2},\malloc}$ is always acyclic.  \footnote{Note that this also holds for the initial allocation.}  We assume that $G_{\sqrt{2},\malloc}$ contains $k$ source agents. For convenience, we also assume that the agents are re-indexed after each update so that agents $1,2,\ldots,k$ are the sources of $G_{\sqrt{2},\malloc}$, and $\valu(\malloc_1) \leq \valu(\malloc_2) \leq \ldots \leq \valu(\malloc_k)$. We define our potential function as 
$
\phi(\malloc) = \big[ \valu(\malloc_1),\valu(\malloc_2),\ldots, \valu(\malloc_k),\infty \big].
$ We designate our algorithm in this section as $\algot$. 

\subsection{Envy Elimination} \label
{sec:eenew}
As we mentioned before, the envy elimination process is initially introduced by Akrami $\etal$ \cite{akrami2022ef2x}. This process aims to eliminate strong envies among agents while preserving essential allocation properties. Here, we propose a simple alternative for the envy elimination process: Given an allocation $\malloc$ with potential strong envies, as long as there exist two agents, $i$ and $j$, where agent $i$ $\sqrt{2}$-strongly envies agent $j$, we identify a good $\good \in \malloc_j$ such that $\sqrt{2}\valu_i(\malloc_i) < \valu_i(\malloc_j \setminus \{\good\})$, and transfer $\good$ from $\malloc_j$ to $\malloc_0$. 

The envy elimination process turns out to be very useful. Given the nature of the process, we know that the resulting allocation is $\invsq$-$\efx$. Interestingly, as we show in Lemma \ref{lem:2new}, this process also guarantees that the value of the potential function does not decrease.

\begin{lemma}\label{lem:2new}
	Let $\malloc$ be a $\frac{\sqrt{2}}{2}$-$\efx$ allocation satisfying Property \ref{prop:2new}, and let $\malloc'$ be the allocation after applying envy elimination. Then, $\malloc'$ satisfies Property \ref{prop:2new}. Furthermore we have $\phi(\malloc) \leq \phi(\malloc')$.  
\end{lemma}
\begin{proof}
	By definition of the process, Property \ref{prop:2new} trivially holds. To show that $\phi(\malloc) \leq \phi(\malloc')$, note that the envy elimination process may involve multiple updates. We show that after each update, the value of $\phi$ does not decrease. Consider an allocation $\malloc$ where, for some agents $i$ and $j$, we have $\sqrt{2}\valu_i(\malloc_i) < \valu_i({\malloc_j / g})$. Let $\malloc''$ be the allocation after the update, which means $\malloc''$ is identical to $\malloc$ except that good $\good$ is transferred from the bundle of agent $j$ to the pool. Note that agent $j$ is neither a source before the update nor becomes a source after, since agent $i$ $\sqrt{2}$-envies agent $j$ both before and after the process. The only change in the source nodes happens when agent $j$ starts to $\sqrt{2}$-envy some source node after the process. Therefore, the set of sources in $G_\malloc$ is a subset of the set of sources $G_{\malloc''}$. Therefore, by definition of $\phi(\cdot)$, we have $\phi(\malloc) \leq \phi(\malloc'')$, and  consequently, $\phi(\malloc) \leq \phi(\malloc')$.
\end{proof}


\input{src/case6new/U1}
\input{src/case6new/U2}
\input{src/case6new/UF}

\label{case6new}

==> src/case6new/U1.tex <==
\subsection{Update Rule 1} \label{aa:1new}
The first rule takes an allocation $\malloc$ as input, and if there exists an agent $i$ with $\rank_i(\malloc) < \sqrt{2}$ and a good $\good \in \malloc_0$ such that good $\good$ is relevant to agent $i$,  we allocate $\good$ to agent $i$. 

\iffalse
\vspace{0.1cm}
\begin{tcolorbox}[colback=white!5,coltitle=white!95!black,colframe=black!95,
	title= \textbf{Update Rule $1$}]
	
	\textbf{Preconditions:}
	\begin{itemize}
		\item $\malloc$ satisfies Property \ref{prop:2}. 
		\item \label{prec_1new}There exists an unallocated good $ \good \in \malloc_{0}$ and an agent $i$ such that $\valu_i(\good) \neq 0$. 	\end{itemize}
	
	\textbf{Update:}
	\begin{itemize}
		\item $\malloc'_j = \begin{cases}
			\malloc_j & j \in [n] \setminus \{i,0\}\\
			\malloc_i \cup \good & j=i \\
			\malloc_0 \setminus \good & j=0
		\end{cases}$ 
		\item Run envy elimination
	\end{itemize}
\end{tcolorbox}
\fi

\begin{lemma}\label{lem:511new}
	Let $\malloc$ be an allocation satisfying Property \ref{prop:2new}, and let $\malloc'$ be the allocation after applying Rule 1. Then $\malloc'$ satisfies Property \ref{prop:2new}. Furthermore, we have $\phi(\malloc) < \phi(\malloc')$.
\end{lemma}
\begin{proof}
	The only agent whose value for her bundle is changed is agent $i$, and the allocated good $\good$ is relevant to agent $i$. Therefore, Property \ref{prop:2new} holds. Furthermore, $\valu(\malloc'_i) > \valu(\malloc_i)$ and  by Lemma \ref{lem:phi} we have $\phi(\malloc) < \phi(\malloc')$. 
\end{proof}

%\begin{observation}
%	Let $\malloc$ be an allocation satisfying Property \ref{prop:2}, and let $\malloc'$ be the allocation after applying Rule 1. Then $\malloc'$ satisfies Property \ref{prop:2}.
%\end{observation}

==> src/case6new/U2.tex <==
\subsection{Update Rule 2} \label{aa:2new}
In the second updating rule, if for some agent $i$,  $\virtualvalue_i(\malloc) < \valu_i(\malloc_0)$, we update the allocation as follows: since Rule 1 is not applicable, we have $\rank_i(\malloc) > \sqrt{2}$. Let $i_1 \rightarrow i_2 \rightarrow \ldots \rightarrow i_k \rightarrow i$ be the rankpath of $i$ in $\malloc$. We shift the allocation through this path, i.e., for every edge $i_v \rightarrow i_u$ in this path, we allocate $\malloc_{i_u}$ to agent $i_v$. We also allocate $\malloc_0[i]$ to $i$, and return the goods in $\malloc_{i_1}$ back to the pool. 

\iffalse
\vspace{0.1cm}
\begin{tcolorbox}[colback=white!5,coltitle=white!95!black,colframe=black!95,
	title= \textbf{Update Rule $2$}]
	
	\textbf{Preconditions:}
	\begin{itemize}
		\item Rule 1 is not applicable. 
		\item $\malloc$ satisfies Property \ref{prop:2new}. 
		\item There exists a path $i_1 \rightarrow i_2 \rightarrow \ldots \rightarrow i_k$ in $G_{\sqrt{2},\malloc}$ such that $i_1$ is a source in $G_{\sqrt{2},\malloc}$ and $\sqrt{2}\valu_{i_k}(\malloc_{i_k}) < \valu_{i_k}(\malloc_0)$. 
	\end{itemize}
	
	\textbf{Update:}
	\begin{itemize}
		\item $\malloc'_j = \begin{cases}
			\malloc_j & j \in [n] \setminus \{0, i_1,i_2,\ldots,i_k\}\\
			\malloc_{i_{l+1}} & j = i_l \mbox{ for } 1 \le l < k\\
			\relevant_{i_k}(\malloc_0) & j = i_k\\
			\malloc_0 \cup \malloc_{i_1} \setminus \relevant_{i_k}(\malloc_0) & j = 0
		\end{cases}$
		\item Run envy elimination
	\end{itemize}
\end{tcolorbox}
\fi

\begin{lemma}\label{lem:521new}
Let $\malloc$ be an allocation satisfying Property \ref{prop:2new}. Assume that Rule 1 is not applicable,  and let $\malloc'$ be the allocation after applying Rule 2. Then, $\malloc'$ satisfies Property \ref{prop:2new}. Furthermore, we have $\phi(\malloc) < \phi(\malloc')$.
\end{lemma}
\begin{proof}
		Given that agent 
		$i$
		selects only relevant goods from the pool, we have $\valu_i(\malloc'_i) = \valu({\malloc'_i})$. Furthermore, according to Lemma \ref{lem:12new}, for every edge $i_1 \rightarrow i_2$ in the path from $j$ to $i$, we have  $\valu_{i_1}(\malloc'_{i_2}) = \valu(\malloc'_{i_2})$. Consequently, Property \ref{prop:2new} remains valid after the update.
		To prove $\phi(\malloc) < \phi(\malloc')$, we utilize Lemma \ref{lem:phinew}. Considering $A,x,x'$ in the statement of Lemma \ref{lem:phinew} we proceed with: 
	\begin{align*}
		A &= \mbox{Agents in the path from $j$ to $i$ } \\
		x &= \min_{i' \in A}(\valu(\alloc_{i'})) = \valu(\malloc_j) \\
		x' &= \min_{i' \in A}(\valu(\alloc'_{i'}))
	\end{align*}
	Also, since for agent $i$, $\valu(\malloc_j) < \invsq\valu(\malloc_i) 
		< \valu(\malloc'_i),
	$
	and for every other agent $k \in A$, $\valu(\malloc_j) < \invsq\valu(\malloc_{k})$, we have $x < x'$.  
	Finally, agent $j$ is a source in $G_{\sqrt{2}, \malloc}$ and therefore, $x = \valu(\malloc_j)$. Thus, all conditions of Lemma \ref{lem:phinew} are satisfied, which implies $\phi(\malloc) < \phi(\malloc')$.
\end{proof}



==> src/case6new/UF.tex <==
\subsection{Final Step} 
When none of Rules 1 and 2 is feasible, we give the entire pool to agent $i$ such that $\rank_i(\malloc) = 1$ ,and terminate the allocation. 
In Theorem \ref{thm:fstepnew} we show  that the resulting allocation is $\frac{\sqrt{2}}{2}$-$\efx$. 

\iffalse
\vspace{0.1cm}
\begin{tcolorbox}[colback=white!5,coltitle=white!95!black,colframe=black!95,
	title= \textbf{Final Step}]
	\textbf{Preconditions:}
	\begin{itemize}
		\item Rule 1, and Rule 2 are not applicable.
		\item $\malloc$ satisfies Property \ref{prop:2new}. 
	\end{itemize}
	\textbf{Update:}
	\begin{itemize}
		\item Suppose agent $i$ with minimum $\valu(\malloc_i)$. 
		\item $\malloc'_j = \begin{cases}
			\malloc_j & j \in [n] \setminus \{i\}\\
			\malloc_j \cup \malloc_0 & j = i
		\end{cases}$
	\end{itemize}
\end{tcolorbox}
\fi

\begin{theorem}\label{thm:fstepnew}
	Suppose that the valuations are restricted additive, and let $\malloc^*$ be the allocation returned by $\algot$. Then, $\malloc^*$ is a $\frac{\sqrt{2}}{2}$-$\efx$ allocation.
\end{theorem}
\begin{proof}
	Let $\malloc$ be the allocation before the final step.
	First, note that $\rank_i(\malloc) < \sqrt{2}$. We prove that after this allocation, no-one will $\sqrt{2}$-envy $\malloc^*_i$. As a contradiction, 
	suppose agent $j$ $\sqrt{2}$-envies agent $i$. Since $\rank_i(\malloc) < \sqrt{2}$, agent $j$ did not $\sqrt{2}$-envy him before the final step. This means that the pool has a non-zero value for agent $j$, and given the fact that Rule 1 was not applicable, $\rank_j(malloc) > \sqrt{2}$. Now, suppose that agent $k = \roott{j}{\malloc}$. We have
	\begin{align*}
		\valu_j(\malloc^*_i) &= \valu(\malloc_i) + \valu_j(\malloc_0) \\
		&\leq  \valu(\malloc_j) + \valu_j(\malloc_0) &\valu(\malloc_i) \leq\valu(\malloc_j)  \\
		&\leq \frac{\sqrt{2}}{2}\valu(\malloc_k)  + \valu_j(\malloc_0) & \mbox{ $k$ has a path to $j$ in }G_{\sqrt{2},\malloc}\\
		&\leq \frac{\sqrt{2}}{2}\valu(\malloc_k)  + \frac{\sqrt{2}}{2}\valu(\malloc_k) & \mbox{$k$ does not $\sqrt{2}$-envy $\malloc_0$}\\
		&\leq \sqrt{2}\valu(\malloc_k). 
	\end{align*}
	But this contradicts the fact that agent $j$ does not $\sqrt{2}$-envy agent $k$ before the final step.
\end{proof} 

==> src/results.tex <==
\section{Our Results and Techniques}
\label{results}


==> src/table.tex <==
\begin{table}
	\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
      & $\good_1$ & $\good_2$ & $\good_3$ & $\good_4$ & $\good_5$ & $\good_6$  & $\good_7$  \\ \hline
$v_1$ & 3 & 3 & 6 & 0 & 0 & 10 & 0  \\ \hline
$v_2$ & 0 & 0 & 0 & 6 & 7 & 10 & 0  \\ \hline
$v_3$ & 3 & 3 & 0 & 6 & 0 & 0  & 10 \\ \hline
$v_4$ & 0 & 0 & 6 & 0 & 7 & 0  & 10 \\ \hline
%\caption{Agents' valuation over goods}
\end{tabular}
\caption{Agents' valuation over goods}
\label{tb:1}
\end{table}

==> src/table_hypergraph.tex <==
\begin{table}
	\centering
	\begin{tabular}{|l|l|l|l|}
		\hline
		& $g_1$ & $g_2$ & $g_3$ \\ \hline
		$v_1$ & 2     & 0     & 0     \\ \hline
		$v_2$ & 1     & 0     & 5     \\ \hline
		$v_3$ & 4     & 3     & 0     \\ \hline
		$v_4$ & 0     & 4     & 0     \\ \hline
	\end{tabular}
	\caption{Agents' valuation over goods for hypergraph example}
	\label{tb:2}
\end{table}
